Verified Approximation Algorithms

We present the first formal verification of approximation algorithms for NP-complete optimization problems: vertex cover, independent set, set cover, center selection, load balancing, and bin packing. We uncover incompletenesses in existing proofs and improve the approximation ratio in one case. All proofs are uniformly invariant based.

==> Approx_LB_Hoare.tex <==
%
\begin{isabellebody}%
\setisabellecontext{Approx{\isacharunderscore}{\kern0pt}LB{\isacharunderscore}{\kern0pt}Hoare}%
%
\isadelimdocument
%
\endisadelimdocument
%
\isatagdocument
%
\isamarkupsection{Load Balancing%
}
\isamarkuptrue%
%
\endisatagdocument
{\isafolddocument}%
%
\isadelimdocument
%
\endisadelimdocument
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
\isacommand{theory}\isamarkupfalse%
\ Approx{\isacharunderscore}{\kern0pt}LB{\isacharunderscore}{\kern0pt}Hoare\isanewline
\ \ \isakeyword{imports}\ Complex{\isacharunderscore}{\kern0pt}Main\ {\isachardoublequoteopen}HOL{\isacharminus}{\kern0pt}Hoare{\isachardot}{\kern0pt}Hoare{\isacharunderscore}{\kern0pt}Logic{\isachardoublequoteclose}\isanewline
\isakeyword{begin}%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\begin{isamarkuptext}%
This is a formalization of the load balancing algorithms and proofs
in the book by Kleinberg and Tardos \cite{KleinbergT06}.%
\end{isamarkuptext}\isamarkuptrue%
\isacommand{hide{\isacharunderscore}{\kern0pt}const}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}\isakeyword{open}{\isacharparenright}{\kern0pt}\ sorted\isanewline
\isanewline
\isanewline
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ sum{\isacharunderscore}{\kern0pt}le{\isacharunderscore}{\kern0pt}card{\isacharunderscore}{\kern0pt}Max{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isasymlbrakk}\ finite\ A{\isacharsemicolon}{\kern0pt}\ A\ {\isasymnoteq}\ {\isacharbraceleft}{\kern0pt}{\isacharbraceright}{\kern0pt}\ {\isasymrbrakk}\ {\isasymLongrightarrow}\ sum\ f\ A\ {\isasymle}\ card\ A\ {\isacharasterisk}{\kern0pt}\ Max\ {\isacharparenleft}{\kern0pt}f\ {\isacharbackquote}{\kern0pt}\ A{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
\isacommand{proof}\isamarkupfalse%
{\isacharparenleft}{\kern0pt}induction\ A\ rule{\isacharcolon}{\kern0pt}\ finite{\isacharunderscore}{\kern0pt}ne{\isacharunderscore}{\kern0pt}induct{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{case}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}singleton\ x{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}case\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\isacommand{next}\isamarkupfalse%
\isanewline
\ \ \isacommand{case}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}insert\ x\ F{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}case\ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}auto\ simp{\isacharcolon}{\kern0pt}\ max{\isacharunderscore}{\kern0pt}def\ order{\isachardot}{\kern0pt}trans{\isacharbrackleft}{\kern0pt}of\ {\isachardoublequoteopen}sum\ f\ F{\isachardoublequoteclose}\ {\isachardoublequoteopen}card\ F\ {\isacharasterisk}{\kern0pt}\ Max\ {\isacharparenleft}{\kern0pt}f\ {\isacharbackquote}{\kern0pt}\ F{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}{\isacharbrackright}{\kern0pt}{\isacharparenright}{\kern0pt}\isanewline
\isacommand{qed}\isamarkupfalse%
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ Max{\isacharunderscore}{\kern0pt}const{\isacharbrackleft}{\kern0pt}simp{\isacharbrackright}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isasymlbrakk}\ finite\ A{\isacharsemicolon}{\kern0pt}\ A\ {\isasymnoteq}\ {\isacharbraceleft}{\kern0pt}{\isacharbraceright}{\kern0pt}\ {\isasymrbrakk}\ {\isasymLongrightarrow}\ Max\ {\isacharparenleft}{\kern0pt}{\isacharparenleft}{\kern0pt}{\isasymlambda}{\isacharunderscore}{\kern0pt}{\isachardot}{\kern0pt}\ c{\isacharparenright}{\kern0pt}\ {\isacharbackquote}{\kern0pt}\ A{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ c{\isachardoublequoteclose}\isanewline
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
\isacommand{using}\isamarkupfalse%
\ Max{\isacharunderscore}{\kern0pt}in\ image{\isacharunderscore}{\kern0pt}is{\isacharunderscore}{\kern0pt}empty\ \isacommand{by}\isamarkupfalse%
\ blast%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{abbreviation}\isamarkupfalse%
\ Max\isactrlsub {\isadigit{0}}\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}nat\ set\ {\isasymRightarrow}\ nat{\isachardoublequoteclose}\ \isakeyword{where}\isanewline
{\isachardoublequoteopen}Max\isactrlsub {\isadigit{0}}\ N\ {\isasymequiv}\ {\isacharparenleft}{\kern0pt}if\ N{\isacharequal}{\kern0pt}{\isacharbraceleft}{\kern0pt}{\isacharbraceright}{\kern0pt}\ then\ {\isadigit{0}}\ else\ Max\ N{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\isanewline
\isacommand{fun}\isamarkupfalse%
\ f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}nat\ {\isasymRightarrow}\ nat{\isacharparenright}{\kern0pt}\ {\isasymRightarrow}\ nat\ {\isasymRightarrow}\ nat{\isachardoublequoteclose}\ \isakeyword{where}\isanewline
\ \ {\isachardoublequoteopen}f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}\ f\ {\isadigit{0}}\ {\isacharequal}{\kern0pt}\ {\isadigit{0}}{\isachardoublequoteclose}\isanewline
{\isacharbar}{\kern0pt}\ {\isachardoublequoteopen}f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}\ f\ {\isacharparenleft}{\kern0pt}Suc\ x{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ max\ {\isacharparenleft}{\kern0pt}f\ {\isacharparenleft}{\kern0pt}Suc\ x{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}\ f\ x{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}{\isacharunderscore}{\kern0pt}equiv{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}\ f\ n\ {\isacharequal}{\kern0pt}\ Max\isactrlsub {\isadigit{0}}\ {\isacharparenleft}{\kern0pt}f\ {\isacharbackquote}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}n{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}induction\ n{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}auto\ simp{\isacharcolon}{\kern0pt}\ not{\isacharunderscore}{\kern0pt}le\ atLeastAtMostSuc{\isacharunderscore}{\kern0pt}conv{\isacharparenright}{\kern0pt}%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}{\isacharunderscore}{\kern0pt}correct{\isacharcolon}{\kern0pt}\isanewline
\ \ {\isachardoublequoteopen}{\isasymforall}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ T\ x\ {\isasymle}\ f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}\ T\ m{\isachardoublequoteclose}\isanewline
\ \ {\isachardoublequoteopen}m\ {\isachargreater}{\kern0pt}\ {\isadigit{0}}\ {\isasymLongrightarrow}\ {\isasymexists}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ T\ x\ {\isacharequal}{\kern0pt}\ f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}\ T\ m{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ \ %
\endisadelimproof
%
\isatagproof
\isacommand{apply}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}induction\ m{\isacharparenright}{\kern0pt}\isanewline
\ \ \ \ \ \isacommand{apply}\isamarkupfalse%
\ simp{\isacharunderscore}{\kern0pt}all\isanewline
\ \ \ \isacommand{apply}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}metis\ atLeastAtMost{\isacharunderscore}{\kern0pt}iff\ le{\isacharunderscore}{\kern0pt}Suc{\isacharunderscore}{\kern0pt}eq\ max{\isachardot}{\kern0pt}cobounded{\isadigit{1}}\ max{\isachardot}{\kern0pt}coboundedI{\isadigit{2}}{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{subgoal}\isamarkupfalse%
\ \isakeyword{for}\ m\ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}cases\ {\isacartoucheopen}m\ {\isacharequal}{\kern0pt}\ {\isadigit{0}}{\isacartoucheclose}{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}auto\ simp{\isacharcolon}{\kern0pt}\ max{\isacharunderscore}{\kern0pt}def{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{done}\isamarkupfalse%
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}{\isacharunderscore}{\kern0pt}mono{\isacharcolon}{\kern0pt}\isanewline
\ \ {\isachardoublequoteopen}y\ {\isasymle}\ T\ x\ {\isasymLongrightarrow}\ f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}\ {\isacharparenleft}{\kern0pt}T\ {\isacharparenleft}{\kern0pt}x\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ y{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\ m\ {\isasymle}\ f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}\ T\ m{\isachardoublequoteclose}\isanewline
\ \ {\isachardoublequoteopen}T\ x\ {\isasymle}\ y\ {\isasymLongrightarrow}\ f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}\ T\ m\ {\isasymle}\ f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}\ {\isacharparenleft}{\kern0pt}T\ {\isacharparenleft}{\kern0pt}x\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ y{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\ m{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}induction\ m{\isacharparenright}{\kern0pt}\ auto%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}{\isacharunderscore}{\kern0pt}out{\isacharunderscore}{\kern0pt}of{\isacharunderscore}{\kern0pt}range\ {\isacharbrackleft}{\kern0pt}simp{\isacharbrackright}{\kern0pt}{\isacharcolon}{\kern0pt}\isanewline
\ \ {\isachardoublequoteopen}x\ {\isasymnotin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}k{\isacharbraceright}{\kern0pt}\ {\isasymLongrightarrow}\ f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}\ {\isacharparenleft}{\kern0pt}T\ {\isacharparenleft}{\kern0pt}x\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ y{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\ k\ {\isacharequal}{\kern0pt}\ f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}\ T\ k{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}induction\ k{\isacharparenright}{\kern0pt}\ auto%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ fun{\isacharunderscore}{\kern0pt}upd{\isacharunderscore}{\kern0pt}f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ {\isachardoublequoteopen}T\ x\ {\isasymle}\ y{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}\ {\isacharparenleft}{\kern0pt}T\ {\isacharparenleft}{\kern0pt}x\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ y{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\ m\ {\isacharequal}{\kern0pt}\ max\ y\ {\isacharparenleft}{\kern0pt}f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}\ T\ m{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{using}\isamarkupfalse%
\ assms\ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}induction\ m{\isacharparenright}{\kern0pt}\ auto%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{locale}\isamarkupfalse%
\ LoadBalancing\ {\isacharequal}{\kern0pt}\ \isanewline
\ \ \isakeyword{fixes}\ t\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}nat\ {\isasymRightarrow}\ nat{\isachardoublequoteclose}\isanewline
\ \ \ \ \isakeyword{and}\ m\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ nat\isanewline
\ \ \ \ \isakeyword{and}\ n\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ nat\isanewline
\ \ \isakeyword{assumes}\ m{\isacharunderscore}{\kern0pt}gt{\isacharunderscore}{\kern0pt}{\isadigit{0}}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}m\ {\isachargreater}{\kern0pt}\ {\isadigit{0}}{\isachardoublequoteclose}\isanewline
\isakeyword{begin}%
\isadelimdocument
%
\endisadelimdocument
%
\isatagdocument
%
\isamarkupsubsection{Formalization of a Correct Load Balancing%
}
\isamarkuptrue%
%
\isamarkupsubsubsection{Definition%
}
\isamarkuptrue%
%
\endisatagdocument
{\isafolddocument}%
%
\isadelimdocument
%
\endisadelimdocument
\isacommand{definition}\isamarkupfalse%
\ lb\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}nat\ {\isasymRightarrow}\ nat{\isacharparenright}{\kern0pt}\ {\isasymRightarrow}\ {\isacharparenleft}{\kern0pt}nat\ {\isasymRightarrow}\ nat\ set{\isacharparenright}{\kern0pt}\ {\isasymRightarrow}\ nat\ {\isasymRightarrow}\ bool{\isachardoublequoteclose}\ \isakeyword{where}\isanewline
\ \ {\isachardoublequoteopen}lb\ T\ A\ j\ {\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isacharparenleft}{\kern0pt}{\isasymforall}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isasymforall}y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ x\ {\isasymnoteq}\ y\ {\isasymlongrightarrow}\ A\ x\ {\isasyminter}\ A\ y\ {\isacharequal}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}\ %
\isamarkupcmt{No job is assigned to more than one machine%
}\isanewline
\ \ \ \ \ \ \ \ \ \ \ \ \ {\isasymand}\ {\isacharparenleft}{\kern0pt}{\isasymUnion}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ A\ x{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}\ %
\isamarkupcmt{Every job is assigned%
}\isanewline
\ \ \ \ \ \ \ \ \ \ \ \ \ {\isasymand}\ {\isacharparenleft}{\kern0pt}{\isasymforall}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymSum}j\ {\isasymin}\ A\ x{\isachardot}{\kern0pt}\ t\ j{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ T\ x{\isacharparenright}{\kern0pt}\ %
\isamarkupcmt{The processing times sum up to the correct load%
}{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\isanewline
\isacommand{abbreviation}\isamarkupfalse%
\ makespan\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}nat\ {\isasymRightarrow}\ nat{\isacharparenright}{\kern0pt}\ {\isasymRightarrow}\ nat{\isachardoublequoteclose}\ \isakeyword{where}\isanewline
\ \ {\isachardoublequoteopen}makespan\ T\ {\isasymequiv}\ f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}\ T\ m{\isachardoublequoteclose}\isanewline
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ makespan{\isacharunderscore}{\kern0pt}def{\isacharprime}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}makespan\ T\ {\isacharequal}{\kern0pt}\ Max\ {\isacharparenleft}{\kern0pt}T\ {\isacharbackquote}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{using}\isamarkupfalse%
\ m{\isacharunderscore}{\kern0pt}gt{\isacharunderscore}{\kern0pt}{\isadigit{0}}\ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}simp\ add{\isacharcolon}{\kern0pt}\ f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}{\isacharunderscore}{\kern0pt}equiv{\isacharparenright}{\kern0pt}%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ makespan{\isacharunderscore}{\kern0pt}correct{\isacharcolon}{\kern0pt}\isanewline
\ \ {\isachardoublequoteopen}{\isasymforall}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ T\ x\ {\isasymle}\ makespan\ T{\isachardoublequoteclose}\isanewline
\ \ {\isachardoublequoteopen}{\isasymexists}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ T\ x\ {\isacharequal}{\kern0pt}\ makespan\ T{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{using}\isamarkupfalse%
\ f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}{\isacharunderscore}{\kern0pt}correct\ m{\isacharunderscore}{\kern0pt}gt{\isacharunderscore}{\kern0pt}{\isadigit{0}}\ \isacommand{by}\isamarkupfalse%
\ auto%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ lbE{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}lb\ T\ A\ j{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}{\isasymforall}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isasymforall}y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ x\ {\isasymnoteq}\ y\ {\isasymlongrightarrow}\ A\ x\ {\isasyminter}\ A\ y\ {\isacharequal}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \ \ \ \ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}{\isasymUnion}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ A\ x{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \ \ \ \ {\isachardoublequoteopen}{\isasymforall}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymSum}y\ {\isasymin}\ A\ x{\isachardot}{\kern0pt}\ t\ y{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ T\ x{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{using}\isamarkupfalse%
\ assms\ \isacommand{unfolding}\isamarkupfalse%
\ lb{\isacharunderscore}{\kern0pt}def\ \isacommand{by}\isamarkupfalse%
\ blast{\isacharplus}{\kern0pt}%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ lbI{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}{\isasymforall}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isasymforall}y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ x\ {\isasymnoteq}\ y\ {\isasymlongrightarrow}\ A\ x\ {\isasyminter}\ A\ y\ {\isacharequal}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \ \ \ \ \ \ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}{\isasymUnion}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ A\ x{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \ \ \ \ \ \ {\isachardoublequoteopen}{\isasymforall}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymSum}y\ {\isasymin}\ A\ x{\isachardot}{\kern0pt}\ t\ y{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ T\ x{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}lb\ T\ A\ j{\isachardoublequoteclose}%
\isadelimproof
\ %
\endisadelimproof
%
\isatagproof
\isacommand{using}\isamarkupfalse%
\ assms\ \isacommand{unfolding}\isamarkupfalse%
\ lb{\isacharunderscore}{\kern0pt}def\ \isacommand{by}\isamarkupfalse%
\ blast%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
\isanewline
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ A{\isacharunderscore}{\kern0pt}lb{\isacharunderscore}{\kern0pt}finite\ {\isacharbrackleft}{\kern0pt}simp{\isacharbrackright}{\kern0pt}{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}lb\ T\ A\ j{\isachardoublequoteclose}\ {\isachardoublequoteopen}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}finite\ {\isacharparenleft}{\kern0pt}A\ x{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}metis\ lbE{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ assms\ finite{\isacharunderscore}{\kern0pt}UN\ finite{\isacharunderscore}{\kern0pt}atLeastAtMost{\isacharparenright}{\kern0pt}%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\begin{isamarkuptext}%
If \isa{A\ x} is pairwise disjoint for all \isa{x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}}, then the the sum over the sums of the
      individual \isa{A\ x} is equal to the sum over the union of all \isa{A\ x}.%
\end{isamarkuptext}\isamarkuptrue%
\isacommand{lemma}\isamarkupfalse%
\ sum{\isacharunderscore}{\kern0pt}sum{\isacharunderscore}{\kern0pt}eq{\isacharunderscore}{\kern0pt}sum{\isacharunderscore}{\kern0pt}Un{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{fixes}\ A\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}nat\ {\isasymRightarrow}\ nat\ set{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}{\isasymforall}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isasymforall}y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ x\ {\isasymnoteq}\ y\ {\isasymlongrightarrow}\ A\ x\ {\isasyminter}\ A\ y\ {\isacharequal}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \ \ \isakeyword{and}\ {\isachardoublequoteopen}{\isasymforall}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ finite\ {\isacharparenleft}{\kern0pt}A\ x{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}{\isasymSum}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymSum}y\ {\isasymin}\ A\ x{\isachardot}{\kern0pt}\ t\ y{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymSum}x\ {\isasymin}\ {\isacharparenleft}{\kern0pt}{\isasymUnion}y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ A\ y{\isacharparenright}{\kern0pt}{\isachardot}{\kern0pt}\ t\ x{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{using}\isamarkupfalse%
\ assms\isanewline
\isacommand{proof}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}induction\ m{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{case}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}Suc\ m{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ FINITE{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}finite\ {\isacharparenleft}{\kern0pt}{\isasymUnion}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ A\ x{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\ {\isachardoublequoteopen}finite\ {\isacharparenleft}{\kern0pt}A\ {\isacharparenleft}{\kern0pt}Suc\ m{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ Suc{\isachardot}{\kern0pt}prems{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ auto\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isasymforall}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ A\ x\ {\isasyminter}\ A\ {\isacharparenleft}{\kern0pt}Suc\ m{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ Suc{\isachardot}{\kern0pt}prems{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ DISJNT{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}{\isasymUnion}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ A\ x{\isacharparenright}{\kern0pt}\ {\isasyminter}\ {\isacharparenleft}{\kern0pt}A\ {\isacharparenleft}{\kern0pt}Suc\ m{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{using}\isamarkupfalse%
\ Union{\isacharunderscore}{\kern0pt}disjoint\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}{\isasymSum}x\ {\isasymin}\ {\isacharparenleft}{\kern0pt}{\isasymUnion}y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ A\ y{\isacharparenright}{\kern0pt}{\isachardot}{\kern0pt}\ t\ x{\isacharparenright}{\kern0pt}\ {\isacharplus}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymSum}x\ {\isasymin}\ A\ {\isacharparenleft}{\kern0pt}Suc\ m{\isacharparenright}{\kern0pt}{\isachardot}{\kern0pt}\ t\ x{\isacharparenright}{\kern0pt}\isanewline
\ \ \ \ \ \ {\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymSum}x\ {\isasymin}\ {\isacharparenleft}{\kern0pt}{\isacharparenleft}{\kern0pt}{\isasymUnion}y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ A\ y{\isacharparenright}{\kern0pt}\ {\isasymunion}\ A\ {\isacharparenleft}{\kern0pt}Suc\ m{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isachardot}{\kern0pt}\ t\ x{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ sum{\isachardot}{\kern0pt}union{\isacharunderscore}{\kern0pt}disjoint{\isacharbrackleft}{\kern0pt}OF\ FINITE\ DISJNT{\isacharcomma}{\kern0pt}\ symmetric{\isacharbrackright}{\kern0pt}\ \isacommand{{\isachardot}{\kern0pt}}\isamarkupfalse%
\isanewline
\ \ \isacommand{also}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymSum}x\ {\isasymin}\ {\isacharparenleft}{\kern0pt}{\isasymUnion}y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}Suc\ m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ A\ y{\isacharparenright}{\kern0pt}{\isachardot}{\kern0pt}\ t\ x{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}metis\ UN{\isacharunderscore}{\kern0pt}insert\ image{\isacharunderscore}{\kern0pt}Suc{\isacharunderscore}{\kern0pt}lessThan\ image{\isacharunderscore}{\kern0pt}insert\ inf{\isacharunderscore}{\kern0pt}sup{\isacharunderscore}{\kern0pt}aci{\isacharparenleft}{\kern0pt}{\isadigit{5}}{\isacharparenright}{\kern0pt}\ lessThan{\isacharunderscore}{\kern0pt}Suc{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{finally}\isamarkupfalse%
\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}case\ \isacommand{using}\isamarkupfalse%
\ Suc\ \isacommand{by}\isamarkupfalse%
\ auto\isanewline
\isacommand{qed}\isamarkupfalse%
\ simp%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\begin{isamarkuptext}%
If \isa{T} and \isa{A} are a correct load balancing for \isa{j} jobs and \isa{m} machines, 
      then the sum of the loads has to be equal to the sum of the processing times of the jobs%
\end{isamarkuptext}\isamarkuptrue%
\isacommand{lemma}\isamarkupfalse%
\ lb{\isacharunderscore}{\kern0pt}impl{\isacharunderscore}{\kern0pt}job{\isacharunderscore}{\kern0pt}sum{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}lb\ T\ A\ j{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}{\isasymSum}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ T\ x{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymSum}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ t\ x{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
\isacommand{proof}\isamarkupfalse%
\ {\isacharminus}{\kern0pt}\isanewline
\ \ \isacommand{note}\isamarkupfalse%
\ lbrules\ {\isacharequal}{\kern0pt}\ lbE{\isacharbrackleft}{\kern0pt}OF\ assms{\isacharbrackright}{\kern0pt}\isanewline
\ \ \isacommand{from}\isamarkupfalse%
\ assms\ \isacommand{have}\isamarkupfalse%
\ FINITE{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isasymforall}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ finite\ {\isacharparenleft}{\kern0pt}A\ x{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}{\isasymSum}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ T\ x{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymSum}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymSum}y\ {\isasymin}\ A\ x{\isachardot}{\kern0pt}\ t\ y{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ lbrules{\isacharparenleft}{\kern0pt}{\isadigit{3}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{also}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymSum}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ t\ x{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ sum{\isacharunderscore}{\kern0pt}sum{\isacharunderscore}{\kern0pt}eq{\isacharunderscore}{\kern0pt}sum{\isacharunderscore}{\kern0pt}Un{\isacharbrackleft}{\kern0pt}OF\ lbrules{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\ FINITE{\isacharbrackright}{\kern0pt}\isanewline
\ \ \ \ \isacommand{unfolding}\isamarkupfalse%
\ lbrules{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ \isacommand{{\isachardot}{\kern0pt}}\isamarkupfalse%
\isanewline
\ \ \isacommand{finally}\isamarkupfalse%
\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}thesis\ \isacommand{{\isachardot}{\kern0pt}}\isamarkupfalse%
\isanewline
\isacommand{qed}\isamarkupfalse%
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimdocument
%
\endisadelimdocument
%
\isatagdocument
%
\isamarkupsubsubsection{Lower Bounds for the Makespan%
}
\isamarkuptrue%
%
\endisatagdocument
{\isafolddocument}%
%
\isadelimdocument
%
\endisadelimdocument
%
\begin{isamarkuptext}%
If \isa{T} and \isa{A} are a correct load balancing for \isa{j} jobs and \isa{m} machines, then the processing time
      of any job \isa{x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}} is a lower bound for the load of some machine \isa{y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}}%
\end{isamarkuptext}\isamarkuptrue%
\isacommand{lemma}\isamarkupfalse%
\ job{\isacharunderscore}{\kern0pt}lower{\isacharunderscore}{\kern0pt}bound{\isacharunderscore}{\kern0pt}machine{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}lb\ T\ A\ j{\isachardoublequoteclose}\ {\isachardoublequoteopen}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}{\isasymexists}y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ t\ x\ {\isasymle}\ T\ y{\isachardoublequoteclose}\isanewline
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
\isacommand{proof}\isamarkupfalse%
\ {\isacharminus}{\kern0pt}\isanewline
\ \ \isacommand{note}\isamarkupfalse%
\ lbrules\ {\isacharequal}{\kern0pt}\ lbE{\isacharbrackleft}{\kern0pt}OF\ assms{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}{\isacharbrackright}{\kern0pt}\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isasymexists}y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ x\ {\isasymin}\ A\ y{\isachardoublequoteclose}\ \isacommand{using}\isamarkupfalse%
\ lbrules{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ assms{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{obtain}\isamarkupfalse%
\ y\ \isakeyword{where}\ y{\isacharunderscore}{\kern0pt}def{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ {\isachardoublequoteopen}x\ {\isasymin}\ A\ y{\isachardoublequoteclose}\ \isacommand{{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}}\isamarkupfalse%
\isanewline
\ \ \isacommand{moreover}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}finite\ {\isacharparenleft}{\kern0pt}A\ y{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{using}\isamarkupfalse%
\ assms{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\ y{\isacharunderscore}{\kern0pt}def{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{ultimately}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}t\ x\ {\isasymle}\ {\isacharparenleft}{\kern0pt}{\isasymSum}x\ {\isasymin}\ A\ y{\isachardot}{\kern0pt}\ t\ x{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{using}\isamarkupfalse%
\ lbrules{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\ member{\isacharunderscore}{\kern0pt}le{\isacharunderscore}{\kern0pt}sum\ \isacommand{by}\isamarkupfalse%
\ fast\isanewline
\ \ \isacommand{also}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharequal}{\kern0pt}\ T\ y{\isachardoublequoteclose}\ \isacommand{using}\isamarkupfalse%
\ lbrules{\isacharparenleft}{\kern0pt}{\isadigit{3}}{\isacharparenright}{\kern0pt}\ y{\isacharunderscore}{\kern0pt}def{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\ \ \isacommand{finally}\isamarkupfalse%
\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}thesis\ \isacommand{using}\isamarkupfalse%
\ y{\isacharunderscore}{\kern0pt}def{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\isacommand{qed}\isamarkupfalse%
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\begin{isamarkuptext}%
As the load of any machine is a lower bound for the makespan, the processing time 
      of any job \isa{x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}} has to also be a lower bound for the makespan.
      Follows from \isa{job{\isacharunderscore}{\kern0pt}lower{\isacharunderscore}{\kern0pt}bound{\isacharunderscore}{\kern0pt}machine} and \isa{makespan{\isacharunderscore}{\kern0pt}correct}.%
\end{isamarkuptext}\isamarkuptrue%
\isacommand{lemma}\isamarkupfalse%
\ job{\isacharunderscore}{\kern0pt}lower{\isacharunderscore}{\kern0pt}bound{\isacharunderscore}{\kern0pt}makespan{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}lb\ T\ A\ j{\isachardoublequoteclose}\ {\isachardoublequoteopen}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}t\ x\ {\isasymle}\ makespan\ T{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}meson\ job{\isacharunderscore}{\kern0pt}lower{\isacharunderscore}{\kern0pt}bound{\isacharunderscore}{\kern0pt}machine{\isacharbrackleft}{\kern0pt}OF\ assms{\isacharbrackright}{\kern0pt}\ makespan{\isacharunderscore}{\kern0pt}correct{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\ le{\isacharunderscore}{\kern0pt}trans{\isacharparenright}{\kern0pt}%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\begin{isamarkuptext}%
The makespan over \isa{j} jobs is a lower bound for the makespan of any correct load balancing for \isa{j} jobs.%
\end{isamarkuptext}\isamarkuptrue%
\isacommand{lemma}\isamarkupfalse%
\ max{\isacharunderscore}{\kern0pt}job{\isacharunderscore}{\kern0pt}lower{\isacharunderscore}{\kern0pt}bound{\isacharunderscore}{\kern0pt}makespan{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}lb\ T\ A\ j{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}Max\isactrlsub {\isadigit{0}}\ {\isacharparenleft}{\kern0pt}t\ {\isacharbackquote}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}\ {\isasymle}\ makespan\ T{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{using}\isamarkupfalse%
\ job{\isacharunderscore}{\kern0pt}lower{\isacharunderscore}{\kern0pt}bound{\isacharunderscore}{\kern0pt}makespan{\isacharbrackleft}{\kern0pt}OF\ assms{\isacharbrackright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ fastforce%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ job{\isacharunderscore}{\kern0pt}dist{\isacharunderscore}{\kern0pt}lower{\isacharunderscore}{\kern0pt}bound{\isacharunderscore}{\kern0pt}makespan{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}lb\ T\ A\ j{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}{\isasymSum}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ t\ x{\isacharparenright}{\kern0pt}\ {\isacharslash}{\kern0pt}\ m\ {\isasymle}\ makespan\ T{\isachardoublequoteclose}\isanewline
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
\isacommand{proof}\isamarkupfalse%
\ {\isacharminus}{\kern0pt}\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}{\isasymSum}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ t\ x{\isacharparenright}{\kern0pt}\ {\isasymle}\ m\ {\isacharasterisk}{\kern0pt}\ makespan\ T{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ assms\ lb{\isacharunderscore}{\kern0pt}impl{\isacharunderscore}{\kern0pt}job{\isacharunderscore}{\kern0pt}sum{\isacharbrackleft}{\kern0pt}symmetric{\isacharbrackright}{\kern0pt}\isanewline
\ \ \ \ \ \ \isakeyword{and}\ sum{\isacharunderscore}{\kern0pt}le{\isacharunderscore}{\kern0pt}card{\isacharunderscore}{\kern0pt}Max{\isacharbrackleft}{\kern0pt}of\ {\isachardoublequoteopen}{\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}{\isacharbrackright}{\kern0pt}\ m{\isacharunderscore}{\kern0pt}gt{\isacharunderscore}{\kern0pt}{\isadigit{0}}\ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}simp\ add{\isacharcolon}{\kern0pt}\ makespan{\isacharunderscore}{\kern0pt}def{\isacharprime}{\kern0pt}{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}real\ {\isacharparenleft}{\kern0pt}{\isasymSum}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ t\ x{\isacharparenright}{\kern0pt}\ {\isasymle}\ real\ m\ {\isacharasterisk}{\kern0pt}\ real\ {\isacharparenleft}{\kern0pt}makespan\ T{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ of{\isacharunderscore}{\kern0pt}nat{\isacharunderscore}{\kern0pt}mono\ \isacommand{by}\isamarkupfalse%
\ fastforce\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}thesis\ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}simp\ add{\isacharcolon}{\kern0pt}\ field{\isacharunderscore}{\kern0pt}simps\ m{\isacharunderscore}{\kern0pt}gt{\isacharunderscore}{\kern0pt}{\isadigit{0}}{\isacharparenright}{\kern0pt}\isanewline
\isacommand{qed}\isamarkupfalse%
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimdocument
%
\endisadelimdocument
%
\isatagdocument
%
\isamarkupsubsection{The Greedy Approximation Algorithm%
}
\isamarkuptrue%
%
\endisatagdocument
{\isafolddocument}%
%
\isadelimdocument
%
\endisadelimdocument
%
\begin{isamarkuptext}%
This function will perform a linear scan from \isa{k\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}} and return the index of the machine with minimum load assuming \isa{m\ {\isachargreater}{\kern0pt}\ {\isadigit{0}}}%
\end{isamarkuptext}\isamarkuptrue%
\isacommand{fun}\isamarkupfalse%
\ min{\isacharunderscore}{\kern0pt}arg\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}nat\ {\isasymRightarrow}\ nat{\isacharparenright}{\kern0pt}\ {\isasymRightarrow}\ nat\ {\isasymRightarrow}\ nat{\isachardoublequoteclose}\ \isakeyword{where}\isanewline
\ \ {\isachardoublequoteopen}min{\isacharunderscore}{\kern0pt}arg\ T\ {\isadigit{0}}\ {\isacharequal}{\kern0pt}\ {\isadigit{1}}{\isachardoublequoteclose}\isanewline
{\isacharbar}{\kern0pt}\ {\isachardoublequoteopen}min{\isacharunderscore}{\kern0pt}arg\ T\ {\isacharparenleft}{\kern0pt}Suc\ x{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\isanewline
\ \ \ {\isacharparenleft}{\kern0pt}let\ k\ {\isacharequal}{\kern0pt}\ min{\isacharunderscore}{\kern0pt}arg\ T\ x\isanewline
\ \ \ \ in\ if\ T\ {\isacharparenleft}{\kern0pt}Suc\ x{\isacharparenright}{\kern0pt}\ {\isacharless}{\kern0pt}\ T\ k\ then\ {\isacharparenleft}{\kern0pt}Suc\ x{\isacharparenright}{\kern0pt}\ else\ k{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ min{\isacharunderscore}{\kern0pt}correct{\isacharcolon}{\kern0pt}\isanewline
\ \ {\isachardoublequoteopen}{\isasymforall}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ T\ {\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ m{\isacharparenright}{\kern0pt}\ {\isasymle}\ T\ x{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}induction\ m{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}auto\ simp{\isacharcolon}{\kern0pt}\ Let{\isacharunderscore}{\kern0pt}def\ le{\isacharunderscore}{\kern0pt}Suc{\isacharunderscore}{\kern0pt}eq{\isacharcomma}{\kern0pt}\ force{\isacharparenright}{\kern0pt}%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ min{\isacharunderscore}{\kern0pt}in{\isacharunderscore}{\kern0pt}range{\isacharcolon}{\kern0pt}\isanewline
\ \ {\isachardoublequoteopen}k\ {\isachargreater}{\kern0pt}\ {\isadigit{0}}\ {\isasymLongrightarrow}\ {\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ k{\isacharparenright}{\kern0pt}\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}k{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}induction\ k{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}auto\ simp{\isacharcolon}{\kern0pt}\ Let{\isacharunderscore}{\kern0pt}def{\isacharcomma}{\kern0pt}\ force{\isacharplus}{\kern0pt}{\isacharparenright}{\kern0pt}%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ add{\isacharunderscore}{\kern0pt}job{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}lb\ T\ A\ j{\isachardoublequoteclose}\ {\isachardoublequoteopen}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}lb\ {\isacharparenleft}{\kern0pt}T\ {\isacharparenleft}{\kern0pt}x\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ T\ x\ {\isacharplus}{\kern0pt}\ t\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}A\ {\isacharparenleft}{\kern0pt}x\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ A\ x\ {\isasymunion}\ {\isacharbraceleft}{\kern0pt}Suc\ j{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ {\isacharparenleft}{\kern0pt}\isakeyword{is}\ {\isacartoucheopen}lb\ {\isacharquery}{\kern0pt}T\ {\isacharquery}{\kern0pt}A\ {\isacharunderscore}{\kern0pt}{\isacartoucheclose}{\isacharparenright}{\kern0pt}\isanewline
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
\isacommand{proof}\isamarkupfalse%
\ {\isacharminus}{\kern0pt}\isanewline
\ \ \isacommand{note}\isamarkupfalse%
\ lbrules\ {\isacharequal}{\kern0pt}\ lbE{\isacharbrackleft}{\kern0pt}OF\ assms{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}{\isacharbrackright}{\kern0pt}\isanewline
\isanewline
\ \ %
\isamarkupcmt{Rule 1: \isa{A{\isacharparenleft}{\kern0pt}x\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ A\ x\ {\isasymunion}\ {\isacharbraceleft}{\kern0pt}Suc\ j{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}} pairwise disjoint%
}\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ NOTIN{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isasymforall}i\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ Suc\ j\ {\isasymnotin}\ A\ i{\isachardoublequoteclose}\ \isacommand{using}\isamarkupfalse%
\ lbrules{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ assms{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ force\isanewline
\ \ \isacommand{with}\isamarkupfalse%
\ lbrules{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isasymforall}i\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ i\ {\isasymnoteq}\ x\ {\isasymlongrightarrow}\ A\ i\ {\isasyminter}\ {\isacharparenleft}{\kern0pt}A\ x\ {\isasymunion}\ {\isacharbraceleft}{\kern0pt}Suc\ j{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ assms{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isadigit{1}}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isasymforall}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isasymforall}y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ x\ {\isasymnoteq}\ y\ {\isasymlongrightarrow}\ {\isacharquery}{\kern0pt}A\ x\ {\isasyminter}\ {\isacharquery}{\kern0pt}A\ y\ {\isacharequal}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ lbrules{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\isanewline
\ \ %
\isamarkupcmt{Rule 2: \isa{A{\isacharparenleft}{\kern0pt}x\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ A\ x\ {\isasymunion}\ {\isacharbraceleft}{\kern0pt}Suc\ j{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}} contains all jobs%
}\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}{\isasymUnion}y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharquery}{\kern0pt}A\ y{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymUnion}y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ A\ y{\isacharparenright}{\kern0pt}\ {\isasymunion}\ {\isacharbraceleft}{\kern0pt}Suc\ j{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ UNION{\isacharunderscore}{\kern0pt}fun{\isacharunderscore}{\kern0pt}upd\ assms{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ auto\isanewline
\ \ \isacommand{also}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}Suc\ j{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{unfolding}\isamarkupfalse%
\ lbrules{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ auto\isanewline
\ \ \isacommand{finally}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isadigit{2}}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}{\isasymUnion}y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharquery}{\kern0pt}A\ y{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}Suc\ j{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{{\isachardot}{\kern0pt}}\isamarkupfalse%
\isanewline
\isanewline
\ \ %
\isamarkupcmt{Rule 3: \isa{A{\isacharparenleft}{\kern0pt}x\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ A\ x\ {\isasymunion}\ {\isacharbraceleft}{\kern0pt}Suc\ j{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}} sums to \isa{T{\isacharparenleft}{\kern0pt}x\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ T\ x\ {\isacharplus}{\kern0pt}\ t\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}}%
}\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}{\isasymSum}i\ {\isasymin}\ {\isacharquery}{\kern0pt}A\ x{\isachardot}{\kern0pt}\ t\ i{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymSum}i\ {\isasymin}\ A\ x\ {\isasymunion}\ {\isacharbraceleft}{\kern0pt}Suc\ j{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ t\ i{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{moreover}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}A\ x\ {\isasyminter}\ {\isacharbraceleft}{\kern0pt}Suc\ j{\isacharbraceright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{using}\isamarkupfalse%
\ NOTIN\ assms{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\ \ \isacommand{moreover}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}finite\ {\isacharparenleft}{\kern0pt}A\ x{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\ {\isachardoublequoteopen}finite\ {\isacharbraceleft}{\kern0pt}Suc\ j{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{using}\isamarkupfalse%
\ assms\ \isacommand{by}\isamarkupfalse%
\ simp{\isacharplus}{\kern0pt}\isanewline
\ \ \isacommand{ultimately}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}{\isasymSum}i\ {\isasymin}\ {\isacharquery}{\kern0pt}A\ x{\isachardot}{\kern0pt}\ t\ i{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymSum}i\ {\isasymin}\ A\ x{\isachardot}{\kern0pt}\ t\ i{\isacharparenright}{\kern0pt}\ {\isacharplus}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymSum}i\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}Suc\ j{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ t\ i{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ sum{\isachardot}{\kern0pt}union{\isacharunderscore}{\kern0pt}disjoint\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{also}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharequal}{\kern0pt}\ T\ x\ {\isacharplus}{\kern0pt}\ t\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{using}\isamarkupfalse%
\ lbrules{\isacharparenleft}{\kern0pt}{\isadigit{3}}{\isacharparenright}{\kern0pt}\ assms{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{finally}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}{\isasymSum}i\ {\isasymin}\ {\isacharquery}{\kern0pt}A\ x{\isachardot}{\kern0pt}\ t\ i{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharquery}{\kern0pt}T\ x{\isachardoublequoteclose}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isadigit{3}}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isasymforall}i\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymSum}j\ {\isasymin}\ {\isacharquery}{\kern0pt}A\ i{\isachardot}{\kern0pt}\ t\ j{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharquery}{\kern0pt}T\ i{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ lbrules{\isacharparenleft}{\kern0pt}{\isadigit{3}}{\isacharparenright}{\kern0pt}\ assms{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\isanewline
\ \ \isacommand{from}\isamarkupfalse%
\ lbI{\isacharbrackleft}{\kern0pt}OF\ {\isadigit{1}}\ {\isadigit{2}}\ {\isadigit{3}}{\isacharbrackright}{\kern0pt}\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}thesis\ \isacommand{{\isachardot}{\kern0pt}}\isamarkupfalse%
\isanewline
\isacommand{qed}\isamarkupfalse%
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ makespan{\isacharunderscore}{\kern0pt}mono{\isacharcolon}{\kern0pt}\isanewline
\ \ {\isachardoublequoteopen}y\ {\isasymle}\ T\ x\ {\isasymLongrightarrow}\ makespan\ {\isacharparenleft}{\kern0pt}T\ {\isacharparenleft}{\kern0pt}x\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ y{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\ {\isasymle}\ makespan\ T{\isachardoublequoteclose}\isanewline
\ \ {\isachardoublequoteopen}T\ x\ {\isasymle}\ y\ {\isasymLongrightarrow}\ makespan\ T\ {\isasymle}\ makespan\ {\isacharparenleft}{\kern0pt}T\ {\isacharparenleft}{\kern0pt}x\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ y{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{using}\isamarkupfalse%
\ f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}{\isacharunderscore}{\kern0pt}mono\ \isacommand{by}\isamarkupfalse%
\ auto%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ smaller{\isacharunderscore}{\kern0pt}optimum{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}lb\ T\ A\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}{\isasymexists}T{\isacharprime}{\kern0pt}\ A{\isacharprime}{\kern0pt}{\isachardot}{\kern0pt}\ lb\ T{\isacharprime}{\kern0pt}\ A{\isacharprime}{\kern0pt}\ j\ {\isasymand}\ makespan\ T{\isacharprime}{\kern0pt}\ {\isasymle}\ makespan\ T{\isachardoublequoteclose}\isanewline
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
\isacommand{proof}\isamarkupfalse%
\ {\isacharminus}{\kern0pt}\isanewline
\ \ \isacommand{note}\isamarkupfalse%
\ lbrules\ {\isacharequal}{\kern0pt}\ lbE{\isacharbrackleft}{\kern0pt}OF\ assms{\isacharbrackright}{\kern0pt}\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isasymexists}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ Suc\ j\ {\isasymin}\ A\ x{\isachardoublequoteclose}\ \isacommand{using}\isamarkupfalse%
\ lbrules{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ auto\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{obtain}\isamarkupfalse%
\ x\ \isakeyword{where}\ x{\isacharunderscore}{\kern0pt}def{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ {\isachardoublequoteopen}Suc\ j\ {\isasymin}\ A\ x{\isachardoublequoteclose}\ \isacommand{{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}}\isamarkupfalse%
\isanewline
\ \ \isacommand{let}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}T\ {\isacharequal}{\kern0pt}\ {\isachardoublequoteopen}T\ {\isacharparenleft}{\kern0pt}x\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ T\ x\ {\isacharminus}{\kern0pt}\ t\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \isacommand{let}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}A\ {\isacharequal}{\kern0pt}\ {\isachardoublequoteopen}A\ {\isacharparenleft}{\kern0pt}x\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ A\ x\ {\isacharminus}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}Suc\ j{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\isanewline
\ \ %
\isamarkupcmt{Rule 1: \isa{A{\isacharparenleft}{\kern0pt}x\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ A\ x\ {\isacharminus}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}Suc\ j{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}} pairwise disjoint%
}\isanewline
\ \ \isacommand{from}\isamarkupfalse%
\ lbrules{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isasymforall}i\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ i\ {\isasymnoteq}\ x\ {\isasymlongrightarrow}\ A\ i\ {\isasyminter}\ {\isacharparenleft}{\kern0pt}A\ x\ {\isacharminus}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}Suc\ j{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ x{\isacharunderscore}{\kern0pt}def{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isadigit{1}}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isasymforall}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isasymforall}y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ x\ {\isasymnoteq}\ y\ {\isasymlongrightarrow}\ {\isacharquery}{\kern0pt}A\ x\ {\isasyminter}\ {\isacharquery}{\kern0pt}A\ y\ {\isacharequal}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ lbrules{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ auto\isanewline
\isanewline
\ \ %
\isamarkupcmt{Rule 2: \isa{A{\isacharparenleft}{\kern0pt}x\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ A\ x\ {\isacharminus}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}Suc\ j{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}} contains all jobs%
}\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ NOTIN{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isasymforall}i\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ i\ {\isasymnoteq}\ x\ {\isasymlongrightarrow}\ Suc\ j\ {\isasymnotin}\ A\ i{\isachardoublequoteclose}\ \isacommand{using}\isamarkupfalse%
\ lbrules{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\ x{\isacharunderscore}{\kern0pt}def\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}{\isasymUnion}y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharquery}{\kern0pt}A\ y{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymUnion}y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ A\ y{\isacharparenright}{\kern0pt}\ {\isacharminus}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}Suc\ j{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ UNION{\isacharunderscore}{\kern0pt}fun{\isacharunderscore}{\kern0pt}upd\ x{\isacharunderscore}{\kern0pt}def\ \isacommand{by}\isamarkupfalse%
\ auto\isanewline
\ \ \isacommand{also}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{unfolding}\isamarkupfalse%
\ lbrules{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ auto\isanewline
\ \ \isacommand{finally}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isadigit{2}}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}{\isasymUnion}y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharquery}{\kern0pt}A\ y{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{{\isachardot}{\kern0pt}}\isamarkupfalse%
\isanewline
\isanewline
\ \ %
\isamarkupcmt{Rule 3: \isa{A{\isacharparenleft}{\kern0pt}x\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ A\ x\ {\isacharminus}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}Suc\ j{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}} sums to \isa{T{\isacharparenleft}{\kern0pt}x\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ T\ x\ {\isacharminus}{\kern0pt}\ t\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}}%
}\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}{\isasymSum}i\ {\isasymin}\ A\ x\ {\isacharminus}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}Suc\ j{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ t\ i{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymSum}i\ {\isasymin}\ A\ x{\isachardot}{\kern0pt}\ t\ i{\isacharparenright}{\kern0pt}\ {\isacharminus}{\kern0pt}\ t\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}simp\ add{\isacharcolon}{\kern0pt}\ sum{\isacharunderscore}{\kern0pt}diff{\isadigit{1}}{\isacharunderscore}{\kern0pt}nat\ x{\isacharunderscore}{\kern0pt}def{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{also}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharequal}{\kern0pt}\ T\ x\ {\isacharminus}{\kern0pt}\ t\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{using}\isamarkupfalse%
\ lbrules{\isacharparenleft}{\kern0pt}{\isadigit{3}}{\isacharparenright}{\kern0pt}\ x{\isacharunderscore}{\kern0pt}def{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{finally}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}{\isasymSum}i\ {\isasymin}\ {\isacharquery}{\kern0pt}A\ x{\isachardot}{\kern0pt}\ t\ i{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharquery}{\kern0pt}T\ x{\isachardoublequoteclose}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isadigit{3}}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isasymforall}i\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymSum}j\ {\isasymin}\ {\isacharquery}{\kern0pt}A\ i{\isachardot}{\kern0pt}\ t\ j{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharquery}{\kern0pt}T\ i{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ lbrules{\isacharparenleft}{\kern0pt}{\isadigit{3}}{\isacharparenright}{\kern0pt}\ x{\isacharunderscore}{\kern0pt}def{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\isanewline
\ \ %
\isamarkupcmt{\isa{makespan} is not larger%
}\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}lb\ {\isacharquery}{\kern0pt}T\ {\isacharquery}{\kern0pt}A\ j\ {\isasymand}\ makespan\ {\isacharquery}{\kern0pt}T\ {\isasymle}\ makespan\ T{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ lbI{\isacharbrackleft}{\kern0pt}OF\ {\isadigit{1}}\ {\isadigit{2}}\ {\isadigit{3}}{\isacharbrackright}{\kern0pt}\ makespan{\isacharunderscore}{\kern0pt}mono{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ force\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}thesis\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\isacommand{qed}\isamarkupfalse%
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\begin{isamarkuptext}%
If the processing time \isa{y} does not contribute to the makespan, we can ignore it.%
\end{isamarkuptext}\isamarkuptrue%
\isacommand{lemma}\isamarkupfalse%
\ remove{\isacharunderscore}{\kern0pt}small{\isacharunderscore}{\kern0pt}job{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}makespan\ {\isacharparenleft}{\kern0pt}T\ {\isacharparenleft}{\kern0pt}x\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ T\ x\ {\isacharplus}{\kern0pt}\ y{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\ {\isasymnoteq}\ T\ x\ {\isacharplus}{\kern0pt}\ y{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ \ \ {\isachardoublequoteopen}makespan\ {\isacharparenleft}{\kern0pt}T\ {\isacharparenleft}{\kern0pt}x\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ T\ x\ {\isacharplus}{\kern0pt}\ y{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ makespan\ T{\isachardoublequoteclose}\isanewline
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
\isacommand{proof}\isamarkupfalse%
\ {\isacharminus}{\kern0pt}\isanewline
\ \ \isacommand{let}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}T\ {\isacharequal}{\kern0pt}\ {\isachardoublequoteopen}T\ {\isacharparenleft}{\kern0pt}x\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ T\ x\ {\isacharplus}{\kern0pt}\ y{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ NOT{\isacharunderscore}{\kern0pt}X{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}makespan\ {\isacharquery}{\kern0pt}T\ {\isasymnoteq}\ {\isacharquery}{\kern0pt}T\ x{\isachardoublequoteclose}\ \isacommand{using}\isamarkupfalse%
\ assms{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isasymexists}i\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ makespan\ {\isacharquery}{\kern0pt}T\ {\isacharequal}{\kern0pt}\ {\isacharquery}{\kern0pt}T\ i\ {\isasymand}\ i\ {\isasymnoteq}\ x{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ makespan{\isacharunderscore}{\kern0pt}correct{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ metis\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{obtain}\isamarkupfalse%
\ i\ \isakeyword{where}\ i{\isacharunderscore}{\kern0pt}def{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}i\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ {\isachardoublequoteopen}makespan\ {\isacharquery}{\kern0pt}T\ {\isacharequal}{\kern0pt}\ {\isacharquery}{\kern0pt}T\ i{\isachardoublequoteclose}\ {\isachardoublequoteopen}i\ {\isasymnoteq}\ x{\isachardoublequoteclose}\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isacharquery}{\kern0pt}T\ i\ {\isacharequal}{\kern0pt}\ T\ i{\isachardoublequoteclose}\ \isacommand{using}\isamarkupfalse%
\ NOT{\isacharunderscore}{\kern0pt}X\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{moreover}\isamarkupfalse%
\ \isacommand{from}\isamarkupfalse%
\ this\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}makespan\ T\ {\isacharequal}{\kern0pt}\ T\ i{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}metis\ i{\isacharunderscore}{\kern0pt}def{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharcomma}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ antisym{\isacharunderscore}{\kern0pt}conv\ le{\isacharunderscore}{\kern0pt}add{\isadigit{1}}\ makespan{\isacharunderscore}{\kern0pt}mono{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ makespan{\isacharunderscore}{\kern0pt}correct{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{ultimately}\isamarkupfalse%
\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}thesis\ \isacommand{using}\isamarkupfalse%
\ i{\isacharunderscore}{\kern0pt}def{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\isacommand{qed}\isamarkupfalse%
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ greedy{\isacharunderscore}{\kern0pt}makespan{\isacharunderscore}{\kern0pt}no{\isacharunderscore}{\kern0pt}jobs\ {\isacharbrackleft}{\kern0pt}simp{\isacharbrackright}{\kern0pt}{\isacharcolon}{\kern0pt}\isanewline
\ \ {\isachardoublequoteopen}makespan\ {\isacharparenleft}{\kern0pt}{\isasymlambda}{\isacharunderscore}{\kern0pt}{\isachardot}{\kern0pt}\ {\isadigit{0}}{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isadigit{0}}{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{using}\isamarkupfalse%
\ m{\isacharunderscore}{\kern0pt}gt{\isacharunderscore}{\kern0pt}{\isadigit{0}}\ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}simp\ add{\isacharcolon}{\kern0pt}\ makespan{\isacharunderscore}{\kern0pt}def{\isacharprime}{\kern0pt}{\isacharparenright}{\kern0pt}%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ min{\isacharunderscore}{\kern0pt}avg{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}m\ {\isacharasterisk}{\kern0pt}\ T\ {\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ m{\isacharparenright}{\kern0pt}\ {\isasymle}\ {\isacharparenleft}{\kern0pt}{\isasymSum}i\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ T\ i{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \ \ \ \ \ \ \ {\isacharparenleft}{\kern0pt}\isakeyword{is}\ {\isacartoucheopen}{\isacharunderscore}{\kern0pt}\ {\isacharasterisk}{\kern0pt}\ {\isacharquery}{\kern0pt}T\ {\isasymle}\ {\isacharquery}{\kern0pt}S{\isacartoucheclose}{\isacharparenright}{\kern0pt}\isanewline
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
\isacommand{proof}\isamarkupfalse%
\ {\isacharminus}{\kern0pt}\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}{\isasymSum}{\isacharunderscore}{\kern0pt}\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharquery}{\kern0pt}T{\isacharparenright}{\kern0pt}\ {\isasymle}\ {\isacharquery}{\kern0pt}S{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ sum{\isacharunderscore}{\kern0pt}mono{\isacharbrackleft}{\kern0pt}of\ {\isacartoucheopen}{\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isacartoucheclose}\ {\isacartoucheopen}{\isasymlambda}{\isacharunderscore}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharquery}{\kern0pt}T{\isacartoucheclose}\ T{\isacharbrackright}{\kern0pt}\isanewline
\ \ \ \ \ \ \isakeyword{and}\ min{\isacharunderscore}{\kern0pt}correct\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}thesis\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\isacommand{qed}\isamarkupfalse%
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{definition}\isamarkupfalse%
\ inv\isactrlsub {\isadigit{1}}\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}nat\ {\isasymRightarrow}\ nat{\isacharparenright}{\kern0pt}\ {\isasymRightarrow}\ {\isacharparenleft}{\kern0pt}nat\ {\isasymRightarrow}\ nat\ set{\isacharparenright}{\kern0pt}\ {\isasymRightarrow}\ nat\ {\isasymRightarrow}\ bool{\isachardoublequoteclose}\ \isakeyword{where}\isanewline
\ \ {\isachardoublequoteopen}inv\isactrlsub {\isadigit{1}}\ T\ A\ j\ {\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}lb\ T\ A\ j\ {\isasymand}\ j\ {\isasymle}\ n\ {\isasymand}\ {\isacharparenleft}{\kern0pt}{\isasymforall}T{\isacharprime}{\kern0pt}\ A{\isacharprime}{\kern0pt}{\isachardot}{\kern0pt}\ lb\ T{\isacharprime}{\kern0pt}\ A{\isacharprime}{\kern0pt}\ j\ {\isasymlongrightarrow}\ makespan\ T\ {\isasymle}\ {\isadigit{2}}\ {\isacharasterisk}{\kern0pt}\ makespan\ T{\isacharprime}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ inv\isactrlsub {\isadigit{1}}E{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}inv\isactrlsub {\isadigit{1}}\ T\ A\ j{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}lb\ T\ A\ j{\isachardoublequoteclose}\ {\isachardoublequoteopen}j\ {\isasymle}\ n{\isachardoublequoteclose}\isanewline
\ \ \ \ \ \ \ \ {\isachardoublequoteopen}lb\ T{\isacharprime}{\kern0pt}\ A{\isacharprime}{\kern0pt}\ j\ {\isasymLongrightarrow}\ makespan\ T\ {\isasymle}\ {\isadigit{2}}\ {\isacharasterisk}{\kern0pt}\ makespan\ T{\isacharprime}{\kern0pt}{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{using}\isamarkupfalse%
\ assms\ \isacommand{unfolding}\isamarkupfalse%
\ inv\isactrlsub {\isadigit{1}}{\isacharunderscore}{\kern0pt}def\ \isacommand{by}\isamarkupfalse%
\ blast{\isacharplus}{\kern0pt}%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ inv\isactrlsub {\isadigit{1}}I{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}lb\ T\ A\ j{\isachardoublequoteclose}\ {\isachardoublequoteopen}j\ {\isasymle}\ n{\isachardoublequoteclose}\ {\isachardoublequoteopen}{\isasymforall}T{\isacharprime}{\kern0pt}\ A{\isacharprime}{\kern0pt}{\isachardot}{\kern0pt}\ lb\ T{\isacharprime}{\kern0pt}\ A{\isacharprime}{\kern0pt}\ j\ {\isasymlongrightarrow}\ makespan\ T\ {\isasymle}\ {\isadigit{2}}\ {\isacharasterisk}{\kern0pt}\ makespan\ T{\isacharprime}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}inv\isactrlsub {\isadigit{1}}\ T\ A\ j{\isachardoublequoteclose}%
\isadelimproof
\ %
\endisadelimproof
%
\isatagproof
\isacommand{using}\isamarkupfalse%
\ assms\ \isacommand{unfolding}\isamarkupfalse%
\ inv\isactrlsub {\isadigit{1}}{\isacharunderscore}{\kern0pt}def\ \isacommand{by}\isamarkupfalse%
\ blast%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
\isanewline
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ inv\isactrlsub {\isadigit{1}}{\isacharunderscore}{\kern0pt}step{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}inv\isactrlsub {\isadigit{1}}\ T\ A\ j{\isachardoublequoteclose}\ {\isachardoublequoteopen}j\ {\isacharless}{\kern0pt}\ n{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}inv\isactrlsub {\isadigit{1}}\ {\isacharparenleft}{\kern0pt}T\ {\isacharparenleft}{\kern0pt}{\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ m{\isacharparenright}{\kern0pt}\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ T\ {\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ m{\isacharparenright}{\kern0pt}\ {\isacharplus}{\kern0pt}\ t\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\isanewline
\ \ \ \ \ \ \ \ \ \ \ \ \ \ {\isacharparenleft}{\kern0pt}A\ {\isacharparenleft}{\kern0pt}{\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ m{\isacharparenright}{\kern0pt}\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ A\ {\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ m{\isacharparenright}{\kern0pt}\ {\isasymunion}\ {\isacharbraceleft}{\kern0pt}Suc\ j{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ {\isacharparenleft}{\kern0pt}\isakeyword{is}\ {\isacartoucheopen}inv\isactrlsub {\isadigit{1}}\ {\isacharquery}{\kern0pt}T\ {\isacharquery}{\kern0pt}A\ {\isacharunderscore}{\kern0pt}{\isacartoucheclose}{\isacharparenright}{\kern0pt}\isanewline
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
\isacommand{proof}\isamarkupfalse%
\ {\isacharminus}{\kern0pt}\isanewline
\ \ \isacommand{note}\isamarkupfalse%
\ invrules\ {\isacharequal}{\kern0pt}\ inv\isactrlsub {\isadigit{1}}E{\isacharbrackleft}{\kern0pt}OF\ assms{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}{\isacharbrackright}{\kern0pt}\isanewline
\ \ %
\isamarkupcmt{Greedy is correct%
}\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ LB{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}lb\ {\isacharquery}{\kern0pt}T\ {\isacharquery}{\kern0pt}A\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ add{\isacharunderscore}{\kern0pt}job{\isacharbrackleft}{\kern0pt}OF\ invrules{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\ min{\isacharunderscore}{\kern0pt}in{\isacharunderscore}{\kern0pt}range{\isacharbrackleft}{\kern0pt}OF\ m{\isacharunderscore}{\kern0pt}gt{\isacharunderscore}{\kern0pt}{\isadigit{0}}{\isacharbrackright}{\kern0pt}{\isacharbrackright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\ \ %
\isamarkupcmt{Greedy maintains approximation factor%
}\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ MK{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isasymforall}T{\isacharprime}{\kern0pt}\ A{\isacharprime}{\kern0pt}{\isachardot}{\kern0pt}\ lb\ T{\isacharprime}{\kern0pt}\ A{\isacharprime}{\kern0pt}\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}\ {\isasymlongrightarrow}\ makespan\ {\isacharquery}{\kern0pt}T\ {\isasymle}\ {\isadigit{2}}\ {\isacharasterisk}{\kern0pt}\ makespan\ T{\isacharprime}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \isacommand{proof}\isamarkupfalse%
\ rule{\isacharplus}{\kern0pt}\isanewline
\ \ \ \ \isacommand{fix}\isamarkupfalse%
\ T\isactrlsub {\isadigit{1}}\ A\isactrlsub {\isadigit{1}}\ \isacommand{assume}\isamarkupfalse%
\ {\isachardoublequoteopen}lb\ T\isactrlsub {\isadigit{1}}\ A\isactrlsub {\isadigit{1}}\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{from}\isamarkupfalse%
\ smaller{\isacharunderscore}{\kern0pt}optimum{\isacharbrackleft}{\kern0pt}OF\ this{\isacharbrackright}{\kern0pt}\isanewline
\ \ \ \ \isacommand{obtain}\isamarkupfalse%
\ T\isactrlsub {\isadigit{0}}\ A\isactrlsub {\isadigit{0}}\ \isakeyword{where}\ {\isachardoublequoteopen}lb\ T\isactrlsub {\isadigit{0}}\ A\isactrlsub {\isadigit{0}}\ j{\isachardoublequoteclose}\ {\isachardoublequoteopen}makespan\ T\isactrlsub {\isadigit{0}}\ {\isasymle}\ makespan\ T\isactrlsub {\isadigit{1}}{\isachardoublequoteclose}\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\ \ \ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ IH{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}makespan\ T\ {\isasymle}\ {\isadigit{2}}\ {\isacharasterisk}{\kern0pt}\ makespan\ T\isactrlsub {\isadigit{1}}{\isachardoublequoteclose}\isanewline
\ \ \ \ \ \ \isacommand{using}\isamarkupfalse%
\ invrules{\isacharparenleft}{\kern0pt}{\isadigit{3}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ force\isanewline
\ \ \ \ \isacommand{show}\isamarkupfalse%
\ {\isachardoublequoteopen}makespan\ {\isacharquery}{\kern0pt}T\ {\isasymle}\ {\isadigit{2}}\ {\isacharasterisk}{\kern0pt}\ makespan\ T\isactrlsub {\isadigit{1}}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{proof}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}cases\ {\isacartoucheopen}makespan\ {\isacharquery}{\kern0pt}T\ {\isacharequal}{\kern0pt}\ T\ {\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ m{\isacharparenright}{\kern0pt}\ {\isacharplus}{\kern0pt}\ t\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isacartoucheclose}{\isacharparenright}{\kern0pt}\isanewline
\ \ \ \ \ \ \isacommand{case}\isamarkupfalse%
\ True\isanewline
\ \ \ \ \ \ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}m\ {\isacharasterisk}{\kern0pt}\ T\ {\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ m{\isacharparenright}{\kern0pt}\ {\isasymle}\ {\isacharparenleft}{\kern0pt}{\isasymSum}i\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ T\ i{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}rule\ min{\isacharunderscore}{\kern0pt}avg{\isacharparenright}{\kern0pt}\isanewline
\ \ \ \ \ \ \isacommand{also}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymSum}i\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ t\ i{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}rule\ lb{\isacharunderscore}{\kern0pt}impl{\isacharunderscore}{\kern0pt}job{\isacharunderscore}{\kern0pt}sum{\isacharbrackleft}{\kern0pt}OF\ invrules{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}{\isacharbrackright}{\kern0pt}{\isacharparenright}{\kern0pt}\isanewline
\ \ \ \ \ \ \isacommand{finally}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}real\ m\ {\isacharasterisk}{\kern0pt}\ T\ {\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ m{\isacharparenright}{\kern0pt}\ {\isasymle}\ {\isacharparenleft}{\kern0pt}{\isasymSum}i\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ t\ i{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \ \ \ \ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}auto\ dest{\isacharcolon}{\kern0pt}\ of{\isacharunderscore}{\kern0pt}nat{\isacharunderscore}{\kern0pt}mono{\isacharparenright}{\kern0pt}\isanewline
\ \ \ \ \ \ \isacommand{with}\isamarkupfalse%
\ m{\isacharunderscore}{\kern0pt}gt{\isacharunderscore}{\kern0pt}{\isadigit{0}}\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}T\ {\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ m{\isacharparenright}{\kern0pt}\ {\isasymle}\ {\isacharparenleft}{\kern0pt}{\isasymSum}i\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ t\ i{\isacharparenright}{\kern0pt}\ {\isacharslash}{\kern0pt}\ m{\isachardoublequoteclose}\isanewline
\ \ \ \ \ \ \ \ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}simp\ add{\isacharcolon}{\kern0pt}\ field{\isacharunderscore}{\kern0pt}simps{\isacharparenright}{\kern0pt}\isanewline
\ \ \ \ \ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}T\ {\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ m{\isacharparenright}{\kern0pt}\ {\isasymle}\ makespan\ T\isactrlsub {\isadigit{1}}{\isachardoublequoteclose}\isanewline
\ \ \ \ \ \ \ \ \isacommand{using}\isamarkupfalse%
\ job{\isacharunderscore}{\kern0pt}dist{\isacharunderscore}{\kern0pt}lower{\isacharunderscore}{\kern0pt}bound{\isacharunderscore}{\kern0pt}makespan{\isacharbrackleft}{\kern0pt}OF\ {\isacartoucheopen}lb\ T\isactrlsub {\isadigit{0}}\ A\isactrlsub {\isadigit{0}}\ j{\isacartoucheclose}{\isacharbrackright}{\kern0pt}\ \isanewline
\ \ \ \ \ \ \ \ \ \ \isakeyword{and}\ {\isacartoucheopen}makespan\ T\isactrlsub {\isadigit{0}}\ {\isasymle}\ makespan\ T\isactrlsub {\isadigit{1}}{\isacartoucheclose}\ \isacommand{by}\isamarkupfalse%
\ linarith\isanewline
\ \ \ \ \ \ \isacommand{moreover}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}t\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}\ {\isasymle}\ makespan\ T\isactrlsub {\isadigit{1}}{\isachardoublequoteclose}\isanewline
\ \ \ \ \ \ \ \ \isacommand{using}\isamarkupfalse%
\ job{\isacharunderscore}{\kern0pt}lower{\isacharunderscore}{\kern0pt}bound{\isacharunderscore}{\kern0pt}makespan{\isacharbrackleft}{\kern0pt}OF\ {\isacartoucheopen}lb\ T\isactrlsub {\isadigit{1}}\ A\isactrlsub {\isadigit{1}}\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isacartoucheclose}{\isacharbrackright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \ \ \ \ \isacommand{ultimately}\isamarkupfalse%
\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}thesis\ \isacommand{unfolding}\isamarkupfalse%
\ True\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \ \ \isacommand{next}\isamarkupfalse%
\isanewline
\ \ \ \ \ \ \isacommand{case}\isamarkupfalse%
\ False\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}thesis\ \isacommand{using}\isamarkupfalse%
\ remove{\isacharunderscore}{\kern0pt}small{\isacharunderscore}{\kern0pt}job{\isacharbrackleft}{\kern0pt}OF\ False{\isacharbrackright}{\kern0pt}\ IH\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \ \ \isacommand{qed}\isamarkupfalse%
\isanewline
\ \ \isacommand{qed}\isamarkupfalse%
\isanewline
\ \ \isacommand{from}\isamarkupfalse%
\ inv\isactrlsub {\isadigit{1}}I{\isacharbrackleft}{\kern0pt}OF\ LB\ {\isacharunderscore}{\kern0pt}\ MK{\isacharbrackright}{\kern0pt}\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}thesis\ \isacommand{using}\isamarkupfalse%
\ assms{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\isacommand{qed}\isamarkupfalse%
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ simple{\isacharunderscore}{\kern0pt}greedy{\isacharunderscore}{\kern0pt}approximation{\isacharcolon}{\kern0pt}\isanewline
{\isachardoublequoteopen}VARS\ T\ A\ i\ j\isanewline
{\isacharbraceleft}{\kern0pt}True{\isacharbraceright}{\kern0pt}\isanewline
T\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymlambda}{\isacharunderscore}{\kern0pt}{\isachardot}{\kern0pt}\ {\isadigit{0}}{\isacharparenright}{\kern0pt}{\isacharsemicolon}{\kern0pt}\isanewline
A\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymlambda}{\isacharunderscore}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharsemicolon}{\kern0pt}\isanewline
j\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ {\isadigit{0}}{\isacharsemicolon}{\kern0pt}\isanewline
WHILE\ j\ {\isacharless}{\kern0pt}\ n\ INV\ {\isacharbraceleft}{\kern0pt}inv\isactrlsub {\isadigit{1}}\ T\ A\ j{\isacharbraceright}{\kern0pt}\ DO\isanewline
\ \ i\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ min{\isacharunderscore}{\kern0pt}arg\ T\ m{\isacharsemicolon}{\kern0pt}\isanewline
\ \ j\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isacharsemicolon}{\kern0pt}\isanewline
\ \ A\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ A\ {\isacharparenleft}{\kern0pt}i\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ A{\isacharparenleft}{\kern0pt}i{\isacharparenright}{\kern0pt}\ {\isasymunion}\ {\isacharbraceleft}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharsemicolon}{\kern0pt}\isanewline
\ \ T\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ T\ {\isacharparenleft}{\kern0pt}i\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ T{\isacharparenleft}{\kern0pt}i{\isacharparenright}{\kern0pt}\ {\isacharplus}{\kern0pt}\ t\ j{\isacharparenright}{\kern0pt}\isanewline
OD\isanewline
{\isacharbraceleft}{\kern0pt}lb\ T\ A\ n\ {\isasymand}\ {\isacharparenleft}{\kern0pt}{\isasymforall}T{\isacharprime}{\kern0pt}\ A{\isacharprime}{\kern0pt}{\isachardot}{\kern0pt}\ lb\ T{\isacharprime}{\kern0pt}\ A{\isacharprime}{\kern0pt}\ n\ {\isasymlongrightarrow}\ makespan\ T\ {\isasymle}\ {\isadigit{2}}\ {\isacharasterisk}{\kern0pt}\ makespan\ T{\isacharprime}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\isanewline
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
\isacommand{proof}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}vcg{\isacharcomma}{\kern0pt}\ goal{\isacharunderscore}{\kern0pt}cases{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{case}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}{\isadigit{1}}\ T\ A\ i\ j{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}case\ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}simp\ add{\isacharcolon}{\kern0pt}\ lb{\isacharunderscore}{\kern0pt}def\ inv\isactrlsub {\isadigit{1}}{\isacharunderscore}{\kern0pt}def{\isacharparenright}{\kern0pt}\isanewline
\isacommand{next}\isamarkupfalse%
\isanewline
\ \ \isacommand{case}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}{\isadigit{2}}\ T\ A\ i\ j{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}case\ \isacommand{using}\isamarkupfalse%
\ inv\isactrlsub {\isadigit{1}}{\isacharunderscore}{\kern0pt}step\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\isacommand{next}\isamarkupfalse%
\isanewline
\ \ \isacommand{case}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}{\isadigit{3}}\ T\ A\ i\ j{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}case\ \isacommand{unfolding}\isamarkupfalse%
\ inv\isactrlsub {\isadigit{1}}{\isacharunderscore}{\kern0pt}def\ \isacommand{by}\isamarkupfalse%
\ force\isanewline
\isacommand{qed}\isamarkupfalse%
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{definition}\isamarkupfalse%
\ sorted\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}nat\ {\isasymRightarrow}\ bool{\isachardoublequoteclose}\ \isakeyword{where}\isanewline
\ \ {\isachardoublequoteopen}sorted\ j\ {\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymforall}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isasymforall}y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}x{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ t\ x\ {\isasymle}\ t\ y{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ sorted{\isacharunderscore}{\kern0pt}smaller\ {\isacharbrackleft}{\kern0pt}simp{\isacharbrackright}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isasymlbrakk}\ sorted\ j{\isacharsemicolon}{\kern0pt}\ j\ {\isasymge}\ j{\isacharprime}{\kern0pt}\ {\isasymrbrakk}\ {\isasymLongrightarrow}\ sorted\ j{\isacharprime}{\kern0pt}{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{unfolding}\isamarkupfalse%
\ sorted{\isacharunderscore}{\kern0pt}def\ \isacommand{by}\isamarkupfalse%
\ simp%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ j{\isacharunderscore}{\kern0pt}gt{\isacharunderscore}{\kern0pt}m{\isacharunderscore}{\kern0pt}pigeonhole{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}lb\ T\ A\ j{\isachardoublequoteclose}\ {\isachardoublequoteopen}j\ {\isachargreater}{\kern0pt}\ m{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}{\isasymexists}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isasymexists}y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isasymexists}z\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ x\ {\isasymnoteq}\ y\ {\isasymand}\ x\ {\isasymin}\ A\ z\ {\isasymand}\ y\ {\isasymin}\ A\ z{\isachardoublequoteclose}\isanewline
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
\isacommand{proof}\isamarkupfalse%
\ {\isacharminus}{\kern0pt}\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isasymforall}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isasymexists}y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ x\ {\isasymin}\ A\ y{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ lbE{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}{\isacharbrackleft}{\kern0pt}OF\ assms{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}{\isacharbrackright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isasymexists}f{\isachardot}{\kern0pt}\ {\isasymforall}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ x\ {\isasymin}\ A\ {\isacharparenleft}{\kern0pt}f\ x{\isacharparenright}{\kern0pt}\ {\isasymand}\ f\ x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{by}\isamarkupfalse%
\ metis\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{obtain}\isamarkupfalse%
\ f\ \isakeyword{where}\ f{\isacharunderscore}{\kern0pt}def{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isasymforall}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ x\ {\isasymin}\ A\ {\isacharparenleft}{\kern0pt}f\ x{\isacharparenright}{\kern0pt}\ {\isasymand}\ f\ x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}}\isamarkupfalse%
\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}card\ {\isacharparenleft}{\kern0pt}f\ {\isacharbackquote}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}\ {\isasymle}\ card\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}meson\ card{\isacharunderscore}{\kern0pt}mono\ finite{\isacharunderscore}{\kern0pt}atLeastAtMost\ image{\isacharunderscore}{\kern0pt}subset{\isacharunderscore}{\kern0pt}iff{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{also}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharless}{\kern0pt}\ card\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{using}\isamarkupfalse%
\ assms{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{finally}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}card\ {\isacharparenleft}{\kern0pt}f\ {\isacharbackquote}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}\ {\isacharless}{\kern0pt}\ card\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{{\isachardot}{\kern0pt}}\isamarkupfalse%
\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isasymnot}\ inj{\isacharunderscore}{\kern0pt}on\ f\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{using}\isamarkupfalse%
\ pigeonhole\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isasymexists}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isasymexists}y\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ x\ {\isasymnoteq}\ y\ {\isasymand}\ f\ x\ {\isacharequal}{\kern0pt}\ f\ y{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{unfolding}\isamarkupfalse%
\ inj{\isacharunderscore}{\kern0pt}on{\isacharunderscore}{\kern0pt}def\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}thesis\ \isacommand{using}\isamarkupfalse%
\ f{\isacharunderscore}{\kern0pt}def\ \isacommand{by}\isamarkupfalse%
\ metis\isanewline
\isacommand{qed}\isamarkupfalse%
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\begin{isamarkuptext}%
If \isa{T} and \isa{A} are a correct load balancing for \isa{j} jobs and \isa{m} machines with \isa{j\ {\isachargreater}{\kern0pt}\ m},
      and the jobs are sorted in descending order, then there exists a machine \isa{x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}}
      whose load is at least twice as large as the processing time of job \isa{j}.%
\end{isamarkuptext}\isamarkuptrue%
\isacommand{lemma}\isamarkupfalse%
\ sorted{\isacharunderscore}{\kern0pt}job{\isacharunderscore}{\kern0pt}lower{\isacharunderscore}{\kern0pt}bound{\isacharunderscore}{\kern0pt}machine{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}lb\ T\ A\ j{\isachardoublequoteclose}\ {\isachardoublequoteopen}j\ {\isachargreater}{\kern0pt}\ m{\isachardoublequoteclose}\ {\isachardoublequoteopen}sorted\ j{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}{\isasymexists}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isadigit{2}}\ {\isacharasterisk}{\kern0pt}\ t\ j\ {\isasymle}\ T\ x{\isachardoublequoteclose}\isanewline
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
\isacommand{proof}\isamarkupfalse%
\ {\isacharminus}{\kern0pt}\isanewline
\ \ %
\isamarkupcmt{Step 1: Obtaining the jobs%
}\isanewline
\ \ \isacommand{note}\isamarkupfalse%
\ lbrules\ {\isacharequal}{\kern0pt}\ lbE{\isacharbrackleft}{\kern0pt}OF\ assms{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}{\isacharbrackright}{\kern0pt}\isanewline
\ \ \isacommand{obtain}\isamarkupfalse%
\ j\isactrlsub {\isadigit{1}}\ j\isactrlsub {\isadigit{2}}\ x\ \isakeyword{where}\ {\isacharasterisk}{\kern0pt}{\isacharcolon}{\kern0pt}\isanewline
\ \ \ \ {\isachardoublequoteopen}j\isactrlsub {\isadigit{1}}\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ {\isachardoublequoteopen}j\isactrlsub {\isadigit{2}}\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ {\isachardoublequoteopen}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ {\isachardoublequoteopen}j\isactrlsub {\isadigit{1}}\ {\isasymnoteq}\ j\isactrlsub {\isadigit{2}}{\isachardoublequoteclose}\ {\isachardoublequoteopen}j\isactrlsub {\isadigit{1}}\ {\isasymin}\ A\ x{\isachardoublequoteclose}\ {\isachardoublequoteopen}j\isactrlsub {\isadigit{2}}\ {\isasymin}\ A\ x{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ j{\isacharunderscore}{\kern0pt}gt{\isacharunderscore}{\kern0pt}m{\isacharunderscore}{\kern0pt}pigeonhole{\isacharbrackleft}{\kern0pt}OF\ assms{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharcomma}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}{\isacharbrackright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\isanewline
\ \ %
\isamarkupcmt{Step 2: Jobs contained in sum%
}\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}finite\ {\isacharparenleft}{\kern0pt}A\ x{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{using}\isamarkupfalse%
\ assms{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\ {\isacharasterisk}{\kern0pt}{\isacharparenleft}{\kern0pt}{\isadigit{3}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ SUM{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}{\isasymSum}i\ {\isasymin}\ A\ x{\isachardot}{\kern0pt}\ t\ i{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ t\ j\isactrlsub {\isadigit{1}}\ {\isacharplus}{\kern0pt}\ t\ j\isactrlsub {\isadigit{2}}\ {\isacharplus}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymSum}i\ {\isasymin}\ A\ x\ {\isacharminus}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}j\isactrlsub {\isadigit{1}}{\isacharbraceright}{\kern0pt}\ {\isacharminus}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}j\isactrlsub {\isadigit{2}}{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ t\ i{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ {\isacharasterisk}{\kern0pt}{\isacharparenleft}{\kern0pt}{\isadigit{4}}{\isacharminus}{\kern0pt}{\isadigit{6}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}simp\ add{\isacharcolon}{\kern0pt}\ sum{\isachardot}{\kern0pt}remove{\isacharparenright}{\kern0pt}\isanewline
\isanewline
\ \ %
\isamarkupcmt{Step 3: Proof of lower bound%
}\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}t\ j\ {\isasymle}\ t\ j\isactrlsub {\isadigit{1}}{\isachardoublequoteclose}\ {\isachardoublequoteopen}t\ j\ {\isasymle}\ t\ j\isactrlsub {\isadigit{2}}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ assms{\isacharparenleft}{\kern0pt}{\isadigit{3}}{\isacharparenright}{\kern0pt}\ {\isacharasterisk}{\kern0pt}{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharminus}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ \isacommand{unfolding}\isamarkupfalse%
\ sorted{\isacharunderscore}{\kern0pt}def\ \isacommand{by}\isamarkupfalse%
\ auto\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isadigit{2}}\ {\isacharasterisk}{\kern0pt}\ t\ j\ {\isasymle}\ t\ j\isactrlsub {\isadigit{1}}\ {\isacharplus}{\kern0pt}\ t\ j\isactrlsub {\isadigit{2}}{\isachardoublequoteclose}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{also}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}\ {\isasymle}\ {\isacharparenleft}{\kern0pt}{\isasymSum}i\ {\isasymin}\ A\ x{\isachardot}{\kern0pt}\ t\ i{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{unfolding}\isamarkupfalse%
\ SUM\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{finally}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isadigit{2}}\ {\isacharasterisk}{\kern0pt}\ t\ j\ {\isasymle}\ T\ x{\isachardoublequoteclose}\ \isacommand{using}\isamarkupfalse%
\ lbrules{\isacharparenleft}{\kern0pt}{\isadigit{3}}{\isacharparenright}{\kern0pt}\ {\isacharasterisk}{\kern0pt}{\isacharparenleft}{\kern0pt}{\isadigit{3}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}thesis\ \isacommand{using}\isamarkupfalse%
\ {\isacharasterisk}{\kern0pt}{\isacharparenleft}{\kern0pt}{\isadigit{3}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\isacommand{qed}\isamarkupfalse%
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\begin{isamarkuptext}%
Reasoning analogous to \isa{job{\isacharunderscore}{\kern0pt}lower{\isacharunderscore}{\kern0pt}bound{\isacharunderscore}{\kern0pt}makespan}.%
\end{isamarkuptext}\isamarkuptrue%
\isacommand{lemma}\isamarkupfalse%
\ sorted{\isacharunderscore}{\kern0pt}job{\isacharunderscore}{\kern0pt}lower{\isacharunderscore}{\kern0pt}bound{\isacharunderscore}{\kern0pt}makespan{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}lb\ T\ A\ j{\isachardoublequoteclose}\ {\isachardoublequoteopen}j\ {\isachargreater}{\kern0pt}\ m{\isachardoublequoteclose}\ {\isachardoublequoteopen}sorted\ j{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}{\isadigit{2}}\ {\isacharasterisk}{\kern0pt}\ t\ j\ {\isasymle}\ makespan\ T{\isachardoublequoteclose}\isanewline
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
\isacommand{proof}\isamarkupfalse%
\ {\isacharminus}{\kern0pt}\isanewline
\ \ \isacommand{obtain}\isamarkupfalse%
\ x\ \isakeyword{where}\ x{\isacharunderscore}{\kern0pt}def{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ {\isachardoublequoteopen}{\isadigit{2}}\ {\isacharasterisk}{\kern0pt}\ t\ j\ {\isasymle}\ T\ x{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ sorted{\isacharunderscore}{\kern0pt}job{\isacharunderscore}{\kern0pt}lower{\isacharunderscore}{\kern0pt}bound{\isacharunderscore}{\kern0pt}machine{\isacharbrackleft}{\kern0pt}OF\ assms{\isacharbrackright}{\kern0pt}\ \isacommand{{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}}\isamarkupfalse%
\isanewline
\ \ \isacommand{with}\isamarkupfalse%
\ makespan{\isacharunderscore}{\kern0pt}correct{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}T\ x\ {\isasymle}\ makespan\ T{\isachardoublequoteclose}\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\ \ \isacommand{with}\isamarkupfalse%
\ x{\isacharunderscore}{\kern0pt}def{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}thesis\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\isacommand{qed}\isamarkupfalse%
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ min{\isacharunderscore}{\kern0pt}zero{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}k{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ {\isachardoublequoteopen}T\ x\ {\isacharequal}{\kern0pt}\ {\isadigit{0}}{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}T\ {\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ k{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isadigit{0}}{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{using}\isamarkupfalse%
\ assms{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\isanewline
\isacommand{proof}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}induction\ k{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{case}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}Suc\ k{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}case\ \isacommand{proof}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}cases\ {\isacartoucheopen}x\ {\isacharequal}{\kern0pt}\ Suc\ k{\isacartoucheclose}{\isacharparenright}{\kern0pt}\isanewline
\ \ \ \ \isacommand{case}\isamarkupfalse%
\ True\isanewline
\ \ \ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}thesis\ \isacommand{using}\isamarkupfalse%
\ assms{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}simp\ add{\isacharcolon}{\kern0pt}\ Let{\isacharunderscore}{\kern0pt}def{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{next}\isamarkupfalse%
\isanewline
\ \ \ \ \isacommand{case}\isamarkupfalse%
\ False\isanewline
\ \ \ \ \isacommand{with}\isamarkupfalse%
\ Suc\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}T\ {\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ k{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isadigit{0}}{\isachardoublequoteclose}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}thesis\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{qed}\isamarkupfalse%
\isanewline
\isacommand{qed}\isamarkupfalse%
\ simp%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ min{\isacharunderscore}{\kern0pt}zero{\isacharunderscore}{\kern0pt}index{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}k{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ {\isachardoublequoteopen}T\ x\ {\isacharequal}{\kern0pt}\ {\isadigit{0}}{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}min{\isacharunderscore}{\kern0pt}arg\ T\ k\ {\isasymle}\ x{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{using}\isamarkupfalse%
\ assms{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\isanewline
\isacommand{proof}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}induction\ k{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{case}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}Suc\ k{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}case\ \isacommand{proof}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}cases\ {\isacartoucheopen}x\ {\isacharequal}{\kern0pt}\ Suc\ k{\isacartoucheclose}{\isacharparenright}{\kern0pt}\isanewline
\ \ \ \ \isacommand{case}\isamarkupfalse%
\ True\isanewline
\ \ \ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}thesis\ \isacommand{using}\isamarkupfalse%
\ min{\isacharunderscore}{\kern0pt}in{\isacharunderscore}{\kern0pt}range{\isacharbrackleft}{\kern0pt}of\ {\isachardoublequoteopen}Suc\ k{\isachardoublequoteclose}{\isacharbrackright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{next}\isamarkupfalse%
\isanewline
\ \ \ \ \isacommand{case}\isamarkupfalse%
\ False\isanewline
\ \ \ \ \isacommand{with}\isamarkupfalse%
\ Suc{\isachardot}{\kern0pt}prems\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}x\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}k{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \ \ \isacommand{from}\isamarkupfalse%
\ min{\isacharunderscore}{\kern0pt}zero{\isacharbrackleft}{\kern0pt}OF\ this{\isacharcomma}{\kern0pt}\ of\ T{\isacharbrackright}{\kern0pt}\ assms{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}\ Suc{\isachardot}{\kern0pt}IH{\isacharbrackleft}{\kern0pt}OF\ this{\isacharbrackright}{\kern0pt}\isanewline
\ \ \ \ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}thesis\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{qed}\isamarkupfalse%
\isanewline
\isacommand{qed}\isamarkupfalse%
\ simp%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{definition}\isamarkupfalse%
\ inv\isactrlsub {\isadigit{2}}\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}nat\ {\isasymRightarrow}\ nat{\isacharparenright}{\kern0pt}\ {\isasymRightarrow}\ {\isacharparenleft}{\kern0pt}nat\ {\isasymRightarrow}\ nat\ set{\isacharparenright}{\kern0pt}\ {\isasymRightarrow}\ nat\ {\isasymRightarrow}\ bool{\isachardoublequoteclose}\ \isakeyword{where}\isanewline
\ \ {\isachardoublequoteopen}inv\isactrlsub {\isadigit{2}}\ T\ A\ j\ {\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}lb\ T\ A\ j\ {\isasymand}\ j\ {\isasymle}\ n\isanewline
\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ {\isasymand}\ {\isacharparenleft}{\kern0pt}{\isasymforall}T{\isacharprime}{\kern0pt}\ A{\isacharprime}{\kern0pt}{\isachardot}{\kern0pt}\ lb\ T{\isacharprime}{\kern0pt}\ A{\isacharprime}{\kern0pt}\ j\ {\isasymlongrightarrow}\ makespan\ T\ {\isasymle}\ {\isadigit{3}}\ {\isacharslash}{\kern0pt}\ {\isadigit{2}}\ {\isacharasterisk}{\kern0pt}\ makespan\ T{\isacharprime}{\kern0pt}{\isacharparenright}{\kern0pt}\ \isanewline
\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ {\isasymand}\ {\isacharparenleft}{\kern0pt}{\isasymforall}x\ {\isachargreater}{\kern0pt}\ j{\isachardot}{\kern0pt}\ T\ x\ {\isacharequal}{\kern0pt}\ {\isadigit{0}}{\isacharparenright}{\kern0pt}\isanewline
\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ {\isasymand}\ {\isacharparenleft}{\kern0pt}j\ {\isasymle}\ m\ {\isasymlongrightarrow}\ makespan\ T\ {\isacharequal}{\kern0pt}\ Max\isactrlsub {\isadigit{0}}\ {\isacharparenleft}{\kern0pt}t\ {\isacharbackquote}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ inv\isactrlsub {\isadigit{2}}E{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}inv\isactrlsub {\isadigit{2}}\ T\ A\ j{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}lb\ T\ A\ j{\isachardoublequoteclose}\ {\isachardoublequoteopen}j\ {\isasymle}\ n{\isachardoublequoteclose}\isanewline
\ \ \ \ \ \ \ \ {\isachardoublequoteopen}lb\ T{\isacharprime}{\kern0pt}\ A{\isacharprime}{\kern0pt}\ j\ {\isasymLongrightarrow}\ makespan\ T\ {\isasymle}\ {\isadigit{3}}\ {\isacharslash}{\kern0pt}\ {\isadigit{2}}\ {\isacharasterisk}{\kern0pt}\ makespan\ T{\isacharprime}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \ \ \ \ {\isachardoublequoteopen}{\isasymforall}x\ {\isachargreater}{\kern0pt}\ j{\isachardot}{\kern0pt}\ T\ x\ {\isacharequal}{\kern0pt}\ {\isadigit{0}}{\isachardoublequoteclose}\ {\isachardoublequoteopen}j\ {\isasymle}\ m\ {\isasymLongrightarrow}\ makespan\ T\ {\isacharequal}{\kern0pt}\ Max\isactrlsub {\isadigit{0}}\ {\isacharparenleft}{\kern0pt}t\ {\isacharbackquote}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{using}\isamarkupfalse%
\ assms\ \isacommand{unfolding}\isamarkupfalse%
\ inv\isactrlsub {\isadigit{2}}{\isacharunderscore}{\kern0pt}def\ \isacommand{by}\isamarkupfalse%
\ blast{\isacharplus}{\kern0pt}%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ inv\isactrlsub {\isadigit{2}}I{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}lb\ T\ A\ j{\isachardoublequoteclose}\ {\isachardoublequoteopen}j\ {\isasymle}\ n{\isachardoublequoteclose}\isanewline
\ \ \ \ \ \ \ \ \ \ {\isachardoublequoteopen}{\isasymforall}T{\isacharprime}{\kern0pt}\ A{\isacharprime}{\kern0pt}{\isachardot}{\kern0pt}\ lb\ T{\isacharprime}{\kern0pt}\ A{\isacharprime}{\kern0pt}\ j\ {\isasymlongrightarrow}\ makespan\ T\ {\isasymle}\ {\isadigit{3}}\ {\isacharslash}{\kern0pt}\ {\isadigit{2}}\ {\isacharasterisk}{\kern0pt}\ makespan\ T{\isacharprime}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \ \ \ \ \ \ {\isachardoublequoteopen}{\isasymforall}x\ {\isachargreater}{\kern0pt}\ j{\isachardot}{\kern0pt}\ T\ x\ {\isacharequal}{\kern0pt}\ {\isadigit{0}}{\isachardoublequoteclose}\isanewline
\ \ \ \ \ \ \ \ \ \ {\isachardoublequoteopen}j\ {\isasymle}\ m\ {\isasymLongrightarrow}\ makespan\ T\ {\isacharequal}{\kern0pt}\ Max\isactrlsub {\isadigit{0}}\ {\isacharparenleft}{\kern0pt}t\ {\isacharbackquote}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}inv\isactrlsub {\isadigit{2}}\ T\ A\ j{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{unfolding}\isamarkupfalse%
\ inv\isactrlsub {\isadigit{2}}{\isacharunderscore}{\kern0pt}def\ \isacommand{using}\isamarkupfalse%
\ assms\ \isacommand{by}\isamarkupfalse%
\ blast%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ inv\isactrlsub {\isadigit{2}}{\isacharunderscore}{\kern0pt}step{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}sorted\ n{\isachardoublequoteclose}\ {\isachardoublequoteopen}inv\isactrlsub {\isadigit{2}}\ T\ A\ j{\isachardoublequoteclose}\ {\isachardoublequoteopen}j\ {\isacharless}{\kern0pt}\ n{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}inv\isactrlsub {\isadigit{2}}\ {\isacharparenleft}{\kern0pt}T\ {\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ m\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ T{\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ m{\isacharparenright}{\kern0pt}\ {\isacharplus}{\kern0pt}\ t{\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\isanewline
\ \ \ \ \ \ \ \ \ \ \ \ \ \ {\isacharparenleft}{\kern0pt}A\ {\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ m\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ A{\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ m{\isacharparenright}{\kern0pt}\ {\isasymunion}\ {\isacharbraceleft}{\kern0pt}Suc\ j{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ {\isacharparenleft}{\kern0pt}\isakeyword{is}\ {\isacartoucheopen}inv\isactrlsub {\isadigit{2}}\ {\isacharquery}{\kern0pt}T\ {\isacharquery}{\kern0pt}A\ {\isacharunderscore}{\kern0pt}{\isacartoucheclose}{\isacharparenright}{\kern0pt}\isanewline
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
\isacommand{proof}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}cases\ {\isacartoucheopen}Suc\ j\ {\isachargreater}{\kern0pt}\ m{\isacartoucheclose}{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{case}\isamarkupfalse%
\ True\ \isacommand{note}\isamarkupfalse%
\ invrules\ {\isacharequal}{\kern0pt}\ inv\isactrlsub {\isadigit{2}}E{\isacharbrackleft}{\kern0pt}OF\ assms{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}{\isacharbrackright}{\kern0pt}\isanewline
\ \ %
\isamarkupcmt{Greedy is correct%
}\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ LB{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}lb\ {\isacharquery}{\kern0pt}T\ {\isacharquery}{\kern0pt}A\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ add{\isacharunderscore}{\kern0pt}job{\isacharbrackleft}{\kern0pt}OF\ invrules{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\ min{\isacharunderscore}{\kern0pt}in{\isacharunderscore}{\kern0pt}range{\isacharbrackleft}{\kern0pt}OF\ m{\isacharunderscore}{\kern0pt}gt{\isacharunderscore}{\kern0pt}{\isadigit{0}}{\isacharbrackright}{\kern0pt}{\isacharbrackright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\ \ %
\isamarkupcmt{Greedy maintains approximation factor%
}\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ MK{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isasymforall}T{\isacharprime}{\kern0pt}\ A{\isacharprime}{\kern0pt}{\isachardot}{\kern0pt}\ lb\ T{\isacharprime}{\kern0pt}\ A{\isacharprime}{\kern0pt}\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}\ {\isasymlongrightarrow}\ makespan\ {\isacharquery}{\kern0pt}T\ {\isasymle}\ {\isadigit{3}}\ {\isacharslash}{\kern0pt}\ {\isadigit{2}}\ {\isacharasterisk}{\kern0pt}\ makespan\ T{\isacharprime}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \isacommand{proof}\isamarkupfalse%
\ rule{\isacharplus}{\kern0pt}\isanewline
\ \ \ \ \isacommand{fix}\isamarkupfalse%
\ T\isactrlsub {\isadigit{1}}\ A\isactrlsub {\isadigit{1}}\ \isacommand{assume}\isamarkupfalse%
\ {\isachardoublequoteopen}lb\ T\isactrlsub {\isadigit{1}}\ A\isactrlsub {\isadigit{1}}\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{from}\isamarkupfalse%
\ smaller{\isacharunderscore}{\kern0pt}optimum{\isacharbrackleft}{\kern0pt}OF\ this{\isacharbrackright}{\kern0pt}\isanewline
\ \ \ \ \isacommand{obtain}\isamarkupfalse%
\ T\isactrlsub {\isadigit{0}}\ A\isactrlsub {\isadigit{0}}\ \isakeyword{where}\ {\isachardoublequoteopen}lb\ T\isactrlsub {\isadigit{0}}\ A\isactrlsub {\isadigit{0}}\ j{\isachardoublequoteclose}\ {\isachardoublequoteopen}makespan\ T\isactrlsub {\isadigit{0}}\ {\isasymle}\ makespan\ T\isactrlsub {\isadigit{1}}{\isachardoublequoteclose}\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\ \ \ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ IH{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}makespan\ T\ {\isasymle}\ {\isadigit{3}}\ {\isacharslash}{\kern0pt}\ {\isadigit{2}}\ {\isacharasterisk}{\kern0pt}\ makespan\ T\isactrlsub {\isadigit{1}}{\isachardoublequoteclose}\isanewline
\ \ \ \ \ \ \isacommand{using}\isamarkupfalse%
\ invrules{\isacharparenleft}{\kern0pt}{\isadigit{3}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ force\isanewline
\ \ \ \ \isacommand{show}\isamarkupfalse%
\ {\isachardoublequoteopen}makespan\ {\isacharquery}{\kern0pt}T\ {\isasymle}\ {\isadigit{3}}\ {\isacharslash}{\kern0pt}\ {\isadigit{2}}\ {\isacharasterisk}{\kern0pt}\ makespan\ T\isactrlsub {\isadigit{1}}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{proof}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}cases\ {\isacartoucheopen}makespan\ {\isacharquery}{\kern0pt}T\ {\isacharequal}{\kern0pt}\ T\ {\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ m{\isacharparenright}{\kern0pt}\ {\isacharplus}{\kern0pt}\ t\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isacartoucheclose}{\isacharparenright}{\kern0pt}\isanewline
\ \ \ \ \ \ \isacommand{case}\isamarkupfalse%
\ True\isanewline
\ \ \ \ \ \ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}m\ {\isacharasterisk}{\kern0pt}\ T\ {\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ m{\isacharparenright}{\kern0pt}\ {\isasymle}\ {\isacharparenleft}{\kern0pt}{\isasymSum}i\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ T\ i{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}rule\ min{\isacharunderscore}{\kern0pt}avg{\isacharparenright}{\kern0pt}\isanewline
\ \ \ \ \ \ \isacommand{also}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymSum}i\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ t\ i{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}rule\ lb{\isacharunderscore}{\kern0pt}impl{\isacharunderscore}{\kern0pt}job{\isacharunderscore}{\kern0pt}sum{\isacharbrackleft}{\kern0pt}OF\ invrules{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}{\isacharbrackright}{\kern0pt}{\isacharparenright}{\kern0pt}\isanewline
\ \ \ \ \ \ \isacommand{finally}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}real\ m\ {\isacharasterisk}{\kern0pt}\ T\ {\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ m{\isacharparenright}{\kern0pt}\ {\isasymle}\ {\isacharparenleft}{\kern0pt}{\isasymSum}i\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ t\ i{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \ \ \ \ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}auto\ dest{\isacharcolon}{\kern0pt}\ of{\isacharunderscore}{\kern0pt}nat{\isacharunderscore}{\kern0pt}mono{\isacharparenright}{\kern0pt}\isanewline
\ \ \ \ \ \ \isacommand{with}\isamarkupfalse%
\ m{\isacharunderscore}{\kern0pt}gt{\isacharunderscore}{\kern0pt}{\isadigit{0}}\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}T\ {\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ m{\isacharparenright}{\kern0pt}\ {\isasymle}\ {\isacharparenleft}{\kern0pt}{\isasymSum}i\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isachardot}{\kern0pt}\ t\ i{\isacharparenright}{\kern0pt}\ {\isacharslash}{\kern0pt}\ m{\isachardoublequoteclose}\isanewline
\ \ \ \ \ \ \ \ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}simp\ add{\isacharcolon}{\kern0pt}\ field{\isacharunderscore}{\kern0pt}simps{\isacharparenright}{\kern0pt}\isanewline
\ \ \ \ \ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}T\ {\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ m{\isacharparenright}{\kern0pt}\ {\isasymle}\ makespan\ T\isactrlsub {\isadigit{1}}{\isachardoublequoteclose}\isanewline
\ \ \ \ \ \ \ \ \isacommand{using}\isamarkupfalse%
\ job{\isacharunderscore}{\kern0pt}dist{\isacharunderscore}{\kern0pt}lower{\isacharunderscore}{\kern0pt}bound{\isacharunderscore}{\kern0pt}makespan{\isacharbrackleft}{\kern0pt}OF\ {\isacartoucheopen}lb\ T\isactrlsub {\isadigit{0}}\ A\isactrlsub {\isadigit{0}}\ j{\isacartoucheclose}{\isacharbrackright}{\kern0pt}\ \isanewline
\ \ \ \ \ \ \ \ \ \ \isakeyword{and}\ {\isacartoucheopen}makespan\ T\isactrlsub {\isadigit{0}}\ {\isasymle}\ makespan\ T\isactrlsub {\isadigit{1}}{\isacartoucheclose}\ \isacommand{by}\isamarkupfalse%
\ linarith\isanewline
\ \ \ \ \ \ \isacommand{moreover}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isadigit{2}}\ {\isacharasterisk}{\kern0pt}\ t\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}\ {\isasymle}\ makespan\ T\isactrlsub {\isadigit{1}}{\isachardoublequoteclose}\isanewline
\ \ \ \ \ \ \ \ \isacommand{using}\isamarkupfalse%
\ sorted{\isacharunderscore}{\kern0pt}job{\isacharunderscore}{\kern0pt}lower{\isacharunderscore}{\kern0pt}bound{\isacharunderscore}{\kern0pt}makespan{\isacharbrackleft}{\kern0pt}OF\ {\isacartoucheopen}lb\ T\isactrlsub {\isadigit{1}}\ A\isactrlsub {\isadigit{1}}\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isacartoucheclose}\ {\isacartoucheopen}Suc\ j\ {\isachargreater}{\kern0pt}\ m{\isacartoucheclose}{\isacharbrackright}{\kern0pt}\isanewline
\ \ \ \ \ \ \ \ \ \ \isakeyword{and}\ assms{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharcomma}{\kern0pt}{\isadigit{3}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \ \ \ \ \isacommand{ultimately}\isamarkupfalse%
\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}thesis\ \isacommand{unfolding}\isamarkupfalse%
\ True\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \ \ \isacommand{next}\isamarkupfalse%
\isanewline
\ \ \ \ \ \ \isacommand{case}\isamarkupfalse%
\ False\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}thesis\ \isacommand{using}\isamarkupfalse%
\ remove{\isacharunderscore}{\kern0pt}small{\isacharunderscore}{\kern0pt}job{\isacharbrackleft}{\kern0pt}OF\ False{\isacharbrackright}{\kern0pt}\ IH\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \ \ \isacommand{qed}\isamarkupfalse%
\isanewline
\ \ \isacommand{qed}\isamarkupfalse%
\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}{\isasymforall}x\ {\isachargreater}{\kern0pt}\ Suc\ j{\isachardot}{\kern0pt}\ {\isacharquery}{\kern0pt}T\ x\ {\isacharequal}{\kern0pt}\ {\isadigit{0}}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ invrules{\isacharparenleft}{\kern0pt}{\isadigit{4}}{\isacharparenright}{\kern0pt}\ min{\isacharunderscore}{\kern0pt}in{\isacharunderscore}{\kern0pt}range{\isacharbrackleft}{\kern0pt}OF\ m{\isacharunderscore}{\kern0pt}gt{\isacharunderscore}{\kern0pt}{\isadigit{0}}{\isacharcomma}{\kern0pt}\ of\ T{\isacharbrackright}{\kern0pt}\ True\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{with}\isamarkupfalse%
\ inv\isactrlsub {\isadigit{2}}I{\isacharbrackleft}{\kern0pt}OF\ LB\ {\isacharunderscore}{\kern0pt}\ MK{\isacharbrackright}{\kern0pt}\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}thesis\ \isacommand{using}\isamarkupfalse%
\ assms{\isacharparenleft}{\kern0pt}{\isadigit{3}}{\isacharparenright}{\kern0pt}\ True\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\isacommand{next}\isamarkupfalse%
\isanewline
\ \ \isacommand{case}\isamarkupfalse%
\ False\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ IN{\isacharunderscore}{\kern0pt}RANGE{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}Suc\ j\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}m{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{note}\isamarkupfalse%
\ invrules\ {\isacharequal}{\kern0pt}\ inv\isactrlsub {\isadigit{2}}E{\isacharbrackleft}{\kern0pt}OF\ assms{\isacharparenleft}{\kern0pt}{\isadigit{2}}{\isacharparenright}{\kern0pt}{\isacharbrackright}{\kern0pt}\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}T\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isadigit{0}}{\isachardoublequoteclose}\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\isanewline
\ \ %
\isamarkupcmt{Greedy is correct%
}\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ LB{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}lb\ {\isacharquery}{\kern0pt}T\ {\isacharquery}{\kern0pt}A\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ add{\isacharunderscore}{\kern0pt}job{\isacharbrackleft}{\kern0pt}OF\ invrules{\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharparenright}{\kern0pt}\ min{\isacharunderscore}{\kern0pt}in{\isacharunderscore}{\kern0pt}range{\isacharbrackleft}{\kern0pt}OF\ m{\isacharunderscore}{\kern0pt}gt{\isacharunderscore}{\kern0pt}{\isadigit{0}}{\isacharbrackright}{\kern0pt}{\isacharbrackright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\isanewline
\ \ %
\isamarkupcmt{Greedy is trivially optimal%
}\isanewline
\ \ \isacommand{from}\isamarkupfalse%
\ IN{\isacharunderscore}{\kern0pt}RANGE\ {\isacartoucheopen}T\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isadigit{0}}{\isacartoucheclose}\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}min{\isacharunderscore}{\kern0pt}arg\ T\ m\ {\isasymle}\ Suc\ j{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ min{\isacharunderscore}{\kern0pt}zero{\isacharunderscore}{\kern0pt}index\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\ \ \isacommand{with}\isamarkupfalse%
\ invrules{\isacharparenleft}{\kern0pt}{\isadigit{4}}{\isacharparenright}{\kern0pt}\ \isacommand{have}\isamarkupfalse%
\ EMPTY{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isasymforall}x\ {\isachargreater}{\kern0pt}\ Suc\ j{\isachardot}{\kern0pt}\ {\isacharquery}{\kern0pt}T\ x\ {\isacharequal}{\kern0pt}\ {\isadigit{0}}{\isachardoublequoteclose}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{from}\isamarkupfalse%
\ IN{\isacharunderscore}{\kern0pt}RANGE\ {\isacartoucheopen}T\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isadigit{0}}{\isacartoucheclose}\ \isacommand{have}\isamarkupfalse%
\ {\isachardoublequoteopen}T\ {\isacharparenleft}{\kern0pt}min{\isacharunderscore}{\kern0pt}arg\ T\ m{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isadigit{0}}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{using}\isamarkupfalse%
\ min{\isacharunderscore}{\kern0pt}zero\ \isacommand{by}\isamarkupfalse%
\ blast\isanewline
\ \ \isacommand{with}\isamarkupfalse%
\ fun{\isacharunderscore}{\kern0pt}upd{\isacharunderscore}{\kern0pt}f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}{\isacharbrackleft}{\kern0pt}OF\ min{\isacharunderscore}{\kern0pt}in{\isacharunderscore}{\kern0pt}range{\isacharbrackleft}{\kern0pt}OF\ m{\isacharunderscore}{\kern0pt}gt{\isacharunderscore}{\kern0pt}{\isadigit{0}}{\isacharbrackright}{\kern0pt}{\isacharbrackright}{\kern0pt}\ invrules{\isacharparenleft}{\kern0pt}{\isadigit{5}}{\isacharparenright}{\kern0pt}\ False\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ TRIV{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}makespan\ {\isacharquery}{\kern0pt}T\ {\isacharequal}{\kern0pt}\ Max\isactrlsub {\isadigit{0}}\ {\isacharparenleft}{\kern0pt}t\ {\isacharbackquote}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isadigit{1}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}Suc\ j{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\ \isacommand{unfolding}\isamarkupfalse%
\ f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}{\isacharunderscore}{\kern0pt}equiv{\isacharbrackleft}{\kern0pt}symmetric{\isacharbrackright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\ \ \isacommand{have}\isamarkupfalse%
\ MK{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isasymforall}T{\isacharprime}{\kern0pt}\ A{\isacharprime}{\kern0pt}{\isachardot}{\kern0pt}\ lb\ T{\isacharprime}{\kern0pt}\ A{\isacharprime}{\kern0pt}\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}\ {\isasymlongrightarrow}\ makespan\ {\isacharquery}{\kern0pt}T\ {\isasymle}\ {\isadigit{3}}\ {\isacharslash}{\kern0pt}\ {\isadigit{2}}\ {\isacharasterisk}{\kern0pt}\ makespan\ T{\isacharprime}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}auto\ simp{\isacharcolon}{\kern0pt}\ TRIV{\isacharbrackleft}{\kern0pt}folded\ f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}{\isacharunderscore}{\kern0pt}equiv{\isacharbrackright}{\kern0pt}\isanewline
\ \ \ \ \ \ \ \ \ \ \ \ dest{\isacharbang}{\kern0pt}{\isacharcolon}{\kern0pt}\ max{\isacharunderscore}{\kern0pt}job{\isacharunderscore}{\kern0pt}lower{\isacharunderscore}{\kern0pt}bound{\isacharunderscore}{\kern0pt}makespan{\isacharbrackleft}{\kern0pt}folded\ f{\isacharunderscore}{\kern0pt}Max\isactrlsub {\isadigit{0}}{\isacharunderscore}{\kern0pt}equiv{\isacharbrackright}{\kern0pt}{\isacharparenright}{\kern0pt}\isanewline
\isanewline
\ \ \isacommand{from}\isamarkupfalse%
\ inv\isactrlsub {\isadigit{2}}I{\isacharbrackleft}{\kern0pt}OF\ LB\ {\isacharunderscore}{\kern0pt}\ MK\ EMPTY\ TRIV{\isacharbrackright}{\kern0pt}\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}thesis\ \isacommand{using}\isamarkupfalse%
\ assms{\isacharparenleft}{\kern0pt}{\isadigit{3}}{\isacharparenright}{\kern0pt}\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\isacommand{qed}\isamarkupfalse%
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ sorted{\isacharunderscore}{\kern0pt}greedy{\isacharunderscore}{\kern0pt}approximation{\isacharcolon}{\kern0pt}\isanewline
{\isachardoublequoteopen}sorted\ n\ {\isasymLongrightarrow}\ VARS\ T\ A\ i\ j\isanewline
{\isacharbraceleft}{\kern0pt}True{\isacharbraceright}{\kern0pt}\isanewline
T\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymlambda}{\isacharunderscore}{\kern0pt}{\isachardot}{\kern0pt}\ {\isadigit{0}}{\isacharparenright}{\kern0pt}{\isacharsemicolon}{\kern0pt}\isanewline
A\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isasymlambda}{\isacharunderscore}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharsemicolon}{\kern0pt}\isanewline
j\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ {\isadigit{0}}{\isacharsemicolon}{\kern0pt}\isanewline
WHILE\ j\ {\isacharless}{\kern0pt}\ n\ INV\ {\isacharbraceleft}{\kern0pt}inv\isactrlsub {\isadigit{2}}\ T\ A\ j{\isacharbraceright}{\kern0pt}\ DO\isanewline
\ \ i\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ min{\isacharunderscore}{\kern0pt}arg\ T\ m{\isacharsemicolon}{\kern0pt}\isanewline
\ \ j\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}Suc\ j{\isacharparenright}{\kern0pt}{\isacharsemicolon}{\kern0pt}\isanewline
\ \ A\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ A\ {\isacharparenleft}{\kern0pt}i\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ A{\isacharparenleft}{\kern0pt}i{\isacharparenright}{\kern0pt}\ {\isasymunion}\ {\isacharbraceleft}{\kern0pt}j{\isacharbraceright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharsemicolon}{\kern0pt}\isanewline
\ \ T\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ T\ {\isacharparenleft}{\kern0pt}i\ {\isacharcolon}{\kern0pt}{\isacharequal}{\kern0pt}\ T{\isacharparenleft}{\kern0pt}i{\isacharparenright}{\kern0pt}\ {\isacharplus}{\kern0pt}\ t\ j{\isacharparenright}{\kern0pt}\isanewline
OD\isanewline
{\isacharbraceleft}{\kern0pt}lb\ T\ A\ n\ {\isasymand}\ {\isacharparenleft}{\kern0pt}{\isasymforall}T{\isacharprime}{\kern0pt}\ A{\isacharprime}{\kern0pt}{\isachardot}{\kern0pt}\ lb\ T{\isacharprime}{\kern0pt}\ A{\isacharprime}{\kern0pt}\ n\ {\isasymlongrightarrow}\ makespan\ T\ {\isasymle}\ {\isadigit{3}}\ {\isacharslash}{\kern0pt}\ {\isadigit{2}}\ {\isacharasterisk}{\kern0pt}\ makespan\ T{\isacharprime}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\isanewline
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
\isacommand{proof}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}vcg{\isacharcomma}{\kern0pt}\ goal{\isacharunderscore}{\kern0pt}cases{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{case}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}{\isadigit{1}}\ T\ A\ i\ j{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}case\ \isacommand{by}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}simp\ add{\isacharcolon}{\kern0pt}\ lb{\isacharunderscore}{\kern0pt}def\ inv\isactrlsub {\isadigit{2}}{\isacharunderscore}{\kern0pt}def{\isacharparenright}{\kern0pt}\isanewline
\isacommand{next}\isamarkupfalse%
\isanewline
\ \ \isacommand{case}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}{\isadigit{2}}\ T\ A\ i\ j{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}case\ \isacommand{using}\isamarkupfalse%
\ inv\isactrlsub {\isadigit{2}}{\isacharunderscore}{\kern0pt}step\ \isacommand{by}\isamarkupfalse%
\ simp\isanewline
\isacommand{next}\isamarkupfalse%
\isanewline
\ \ \isacommand{case}\isamarkupfalse%
\ {\isacharparenleft}{\kern0pt}{\isadigit{3}}\ T\ A\ i\ j{\isacharparenright}{\kern0pt}\isanewline
\ \ \isacommand{then}\isamarkupfalse%
\ \isacommand{show}\isamarkupfalse%
\ {\isacharquery}{\kern0pt}case\ \isacommand{unfolding}\isamarkupfalse%
\ inv\isactrlsub {\isadigit{2}}{\isacharunderscore}{\kern0pt}def\ \isacommand{by}\isamarkupfalse%
\ force\isanewline
\isacommand{qed}\isamarkupfalse%
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{end}\isamarkupfalse%
\ \isanewline
%
\isadelimtheory
\isanewline
%
\endisadelimtheory
%
\isatagtheory
\isacommand{end}\isamarkupfalse%
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
\ %
\end{isabellebody}%
\endinput
%:%file=~/Productions/articles/ijcar2020/LMCS/Approx_LB_Hoare.thy%:%
%:%11=1%:%
%:%27=3%:%
%:%28=3%:%
%:%29=4%:%
%:%30=5%:%
%:%39=7%:%
%:%40=8%:%
%:%42=10%:%
%:%43=10%:%
%:%44=11%:%
%:%45=12%:%
%:%46=13%:%
%:%47=14%:%
%:%48=14%:%
%:%55=15%:%
%:%56=15%:%
%:%57=16%:%
%:%58=16%:%
%:%59=17%:%
%:%60=17%:%
%:%61=17%:%
%:%62=17%:%
%:%63=18%:%
%:%64=18%:%
%:%65=19%:%
%:%66=19%:%
%:%67=20%:%
%:%68=20%:%
%:%69=20%:%
%:%70=20%:%
%:%71=21%:%
%:%77=21%:%
%:%80=22%:%
%:%81=23%:%
%:%82=23%:%
%:%89=24%:%
%:%90=24%:%
%:%91=24%:%
%:%96=24%:%
%:%99=25%:%
%:%100=26%:%
%:%101=26%:%
%:%102=27%:%
%:%103=28%:%
%:%104=29%:%
%:%105=29%:%
%:%106=30%:%
%:%107=31%:%
%:%108=32%:%
%:%109=33%:%
%:%110=33%:%
%:%113=34%:%
%:%117=34%:%
%:%118=34%:%
%:%123=34%:%
%:%126=35%:%
%:%127=36%:%
%:%128=36%:%
%:%129=37%:%
%:%130=38%:%
%:%133=39%:%
%:%137=39%:%
%:%138=39%:%
%:%139=40%:%
%:%140=40%:%
%:%141=41%:%
%:%142=41%:%
%:%143=42%:%
%:%144=42%:%
%:%145=42%:%
%:%146=43%:%
%:%152=43%:%
%:%155=44%:%
%:%156=45%:%
%:%157=45%:%
%:%158=46%:%
%:%159=47%:%
%:%162=48%:%
%:%166=48%:%
%:%167=48%:%
%:%172=48%:%
%:%175=49%:%
%:%176=50%:%
%:%177=50%:%
%:%178=51%:%
%:%181=52%:%
%:%185=52%:%
%:%186=52%:%
%:%191=52%:%
%:%194=53%:%
%:%195=54%:%
%:%196=54%:%
%:%197=55%:%
%:%198=56%:%
%:%201=57%:%
%:%205=57%:%
%:%206=57%:%
%:%207=57%:%
%:%212=57%:%
%:%215=58%:%
%:%216=59%:%
%:%217=59%:%
%:%218=60%:%
%:%219=61%:%
%:%220=62%:%
%:%221=63%:%
%:%222=64%:%
%:%229=66%:%
%:%233=68%:%
%:%243=70%:%
%:%244=70%:%
%:%245=71%:%
%:%246=71%:%
%:%247=71%:%
%:%249=72%:%
%:%250=72%:%
%:%252=73%:%
%:%253=73%:%
%:%254=74%:%
%:%255=75%:%
%:%256=75%:%
%:%257=76%:%
%:%258=77%:%
%:%259=78%:%
%:%260=78%:%
%:%263=79%:%
%:%267=79%:%
%:%268=79%:%
%:%269=79%:%
%:%274=79%:%
%:%277=95%:%
%:%278=96%:%
%:%279=97%:%
%:%280=97%:%
%:%281=98%:%
%:%282=99%:%
%:%285=100%:%
%:%289=100%:%
%:%290=100%:%
%:%291=100%:%
%:%296=100%:%
%:%299=101%:%
%:%300=102%:%
%:%301=102%:%
%:%302=103%:%
%:%303=104%:%
%:%304=105%:%
%:%305=106%:%
%:%308=107%:%
%:%312=107%:%
%:%313=107%:%
%:%314=107%:%
%:%315=107%:%
%:%320=107%:%
%:%323=108%:%
%:%324=109%:%
%:%325=109%:%
%:%326=110%:%
%:%327=111%:%
%:%328=112%:%
%:%329=113%:%
%:%331=113%:%
%:%335=113%:%
%:%336=113%:%
%:%337=113%:%
%:%338=113%:%
%:%345=113%:%
%:%346=114%:%
%:%347=115%:%
%:%348=115%:%
%:%349=116%:%
%:%350=117%:%
%:%353=118%:%
%:%357=118%:%
%:%358=118%:%
%:%367=120%:%
%:%368=121%:%
%:%370=122%:%
%:%371=122%:%
%:%372=123%:%
%:%373=124%:%
%:%374=125%:%
%:%375=126%:%
%:%378=127%:%
%:%382=127%:%
%:%383=127%:%
%:%384=128%:%
%:%385=128%:%
%:%386=129%:%
%:%387=129%:%
%:%388=130%:%
%:%389=130%:%
%:%390=131%:%
%:%391=131%:%
%:%392=131%:%
%:%393=132%:%
%:%394=132%:%
%:%395=133%:%
%:%396=133%:%
%:%397=133%:%
%:%398=134%:%
%:%399=134%:%
%:%400=134%:%
%:%401=134%:%
%:%402=134%:%
%:%403=135%:%
%:%404=135%:%
%:%405=136%:%
%:%406=137%:%
%:%407=137%:%
%:%408=137%:%
%:%409=138%:%
%:%410=138%:%
%:%411=138%:%
%:%412=139%:%
%:%413=139%:%
%:%414=140%:%
%:%415=140%:%
%:%416=140%:%
%:%417=140%:%
%:%418=140%:%
%:%419=141%:%
%:%420=141%:%
%:%429=143%:%
%:%430=144%:%
%:%432=145%:%
%:%433=145%:%
%:%434=146%:%
%:%435=147%:%
%:%442=148%:%
%:%443=148%:%
%:%444=149%:%
%:%445=149%:%
%:%446=150%:%
%:%447=150%:%
%:%448=150%:%
%:%449=150%:%
%:%450=151%:%
%:%451=151%:%
%:%452=152%:%
%:%453=152%:%
%:%454=152%:%
%:%455=153%:%
%:%456=153%:%
%:%457=153%:%
%:%458=154%:%
%:%459=154%:%
%:%460=155%:%
%:%461=155%:%
%:%462=155%:%
%:%463=156%:%
%:%464=156%:%
%:%465=156%:%
%:%466=156%:%
%:%467=157%:%
%:%482=159%:%
%:%494=161%:%
%:%495=162%:%
%:%497=163%:%
%:%498=163%:%
%:%499=164%:%
%:%500=165%:%
%:%507=166%:%
%:%508=166%:%
%:%509=167%:%
%:%510=167%:%
%:%511=168%:%
%:%512=168%:%
%:%513=168%:%
%:%514=168%:%
%:%515=169%:%
%:%516=169%:%
%:%517=169%:%
%:%518=169%:%
%:%519=170%:%
%:%520=170%:%
%:%521=170%:%
%:%522=170%:%
%:%523=170%:%
%:%524=171%:%
%:%525=171%:%
%:%526=171%:%
%:%527=171%:%
%:%528=171%:%
%:%529=172%:%
%:%530=172%:%
%:%531=172%:%
%:%532=172%:%
%:%533=172%:%
%:%534=173%:%
%:%535=173%:%
%:%536=173%:%
%:%537=173%:%
%:%538=173%:%
%:%539=174%:%
%:%549=176%:%
%:%550=177%:%
%:%551=178%:%
%:%553=179%:%
%:%554=179%:%
%:%555=180%:%
%:%556=181%:%
%:%559=182%:%
%:%563=182%:%
%:%564=182%:%
%:%573=184%:%
%:%575=185%:%
%:%576=185%:%
%:%577=186%:%
%:%578=187%:%
%:%581=188%:%
%:%585=188%:%
%:%586=188%:%
%:%587=188%:%
%:%592=188%:%
%:%595=189%:%
%:%596=190%:%
%:%597=190%:%
%:%598=191%:%
%:%599=192%:%
%:%606=193%:%
%:%607=193%:%
%:%608=194%:%
%:%609=194%:%
%:%610=195%:%
%:%611=195%:%
%:%612=196%:%
%:%613=196%:%
%:%614=197%:%
%:%615=197%:%
%:%616=197%:%
%:%617=198%:%
%:%618=198%:%
%:%619=198%:%
%:%620=199%:%
%:%621=199%:%
%:%622=199%:%
%:%623=199%:%
%:%624=200%:%
%:%639=202%:%
%:%651=204%:%
%:%653=205%:%
%:%654=205%:%
%:%655=206%:%
%:%656=207%:%
%:%658=209%:%
%:%659=210%:%
%:%660=211%:%
%:%661=211%:%
%:%662=212%:%
%:%665=213%:%
%:%669=213%:%
%:%670=213%:%
%:%675=213%:%
%:%678=214%:%
%:%679=215%:%
%:%680=215%:%
%:%681=216%:%
%:%684=217%:%
%:%688=217%:%
%:%689=217%:%
%:%694=217%:%
%:%697=218%:%
%:%698=219%:%
%:%699=219%:%
%:%700=220%:%
%:%701=221%:%
%:%702=222%:%
%:%709=223%:%
%:%710=223%:%
%:%711=224%:%
%:%712=224%:%
%:%713=225%:%
%:%714=226%:%
%:%715=226%:%
%:%716=226%:%
%:%717=227%:%
%:%718=227%:%
%:%719=227%:%
%:%720=227%:%
%:%721=228%:%
%:%722=228%:%
%:%723=228%:%
%:%724=229%:%
%:%725=229%:%
%:%726=229%:%
%:%727=230%:%
%:%728=230%:%
%:%729=230%:%
%:%730=231%:%
%:%731=231%:%
%:%732=231%:%
%:%733=232%:%
%:%734=233%:%
%:%735=233%:%
%:%736=233%:%
%:%737=234%:%
%:%738=234%:%
%:%739=235%:%
%:%740=235%:%
%:%741=235%:%
%:%742=236%:%
%:%743=236%:%
%:%744=236%:%
%:%745=236%:%
%:%746=236%:%
%:%747=237%:%
%:%748=237%:%
%:%749=237%:%
%:%750=237%:%
%:%751=238%:%
%:%752=239%:%
%:%753=239%:%
%:%754=239%:%
%:%755=240%:%
%:%756=240%:%
%:%757=240%:%
%:%758=241%:%
%:%759=241%:%
%:%760=241%:%
%:%761=241%:%
%:%762=241%:%
%:%763=242%:%
%:%764=242%:%
%:%765=242%:%
%:%766=242%:%
%:%767=242%:%
%:%768=243%:%
%:%769=243%:%
%:%770=243%:%
%:%771=244%:%
%:%772=244%:%
%:%773=244%:%
%:%774=245%:%
%:%775=245%:%
%:%776=245%:%
%:%777=245%:%
%:%778=245%:%
%:%779=246%:%
%:%780=246%:%
%:%781=246%:%
%:%782=246%:%
%:%783=247%:%
%:%784=247%:%
%:%785=247%:%
%:%786=248%:%
%:%787=248%:%
%:%788=248%:%
%:%789=249%:%
%:%790=250%:%
%:%791=250%:%
%:%792=250%:%
%:%793=250%:%
%:%794=251%:%
%:%800=251%:%
%:%803=252%:%
%:%804=253%:%
%:%805=253%:%
%:%806=254%:%
%:%807=255%:%
%:%810=256%:%
%:%814=256%:%
%:%815=256%:%
%:%816=256%:%
%:%821=256%:%
%:%824=257%:%
%:%825=258%:%
%:%826=258%:%
%:%827=259%:%
%:%828=260%:%
%:%835=261%:%
%:%836=261%:%
%:%837=262%:%
%:%838=262%:%
%:%839=263%:%
%:%840=263%:%
%:%841=263%:%
%:%842=263%:%
%:%843=264%:%
%:%844=264%:%
%:%845=264%:%
%:%846=264%:%
%:%847=265%:%
%:%848=265%:%
%:%849=266%:%
%:%850=266%:%
%:%851=267%:%
%:%852=268%:%
%:%853=268%:%
%:%854=268%:%
%:%855=269%:%
%:%856=269%:%
%:%857=269%:%
%:%858=270%:%
%:%859=270%:%
%:%860=270%:%
%:%861=271%:%
%:%862=271%:%
%:%863=271%:%
%:%864=272%:%
%:%865=272%:%
%:%866=272%:%
%:%867=273%:%
%:%868=274%:%
%:%869=274%:%
%:%870=274%:%
%:%871=275%:%
%:%872=275%:%
%:%873=275%:%
%:%874=275%:%
%:%875=276%:%
%:%876=276%:%
%:%877=276%:%
%:%878=277%:%
%:%879=277%:%
%:%880=277%:%
%:%881=278%:%
%:%882=278%:%
%:%883=278%:%
%:%884=278%:%
%:%885=278%:%
%:%886=279%:%
%:%887=279%:%
%:%888=279%:%
%:%889=279%:%
%:%890=280%:%
%:%891=281%:%
%:%892=281%:%
%:%893=281%:%
%:%894=282%:%
%:%895=282%:%
%:%896=283%:%
%:%897=283%:%
%:%898=284%:%
%:%899=284%:%
%:%900=284%:%
%:%901=284%:%
%:%902=284%:%
%:%903=285%:%
%:%904=285%:%
%:%905=285%:%
%:%906=285%:%
%:%907=286%:%
%:%908=286%:%
%:%909=286%:%
%:%910=287%:%
%:%911=287%:%
%:%912=287%:%
%:%913=288%:%
%:%914=289%:%
%:%915=289%:%
%:%916=289%:%
%:%917=290%:%
%:%918=290%:%
%:%919=291%:%
%:%920=291%:%
%:%921=291%:%
%:%922=292%:%
%:%923=292%:%
%:%924=292%:%
%:%925=292%:%
%:%926=293%:%
%:%936=295%:%
%:%938=296%:%
%:%939=296%:%
%:%940=297%:%
%:%941=298%:%
%:%948=299%:%
%:%949=299%:%
%:%950=300%:%
%:%951=300%:%
%:%952=301%:%
%:%953=301%:%
%:%954=301%:%
%:%955=301%:%
%:%956=302%:%
%:%957=302%:%
%:%958=302%:%
%:%959=303%:%
%:%960=303%:%
%:%961=303%:%
%:%962=304%:%
%:%963=304%:%
%:%964=304%:%
%:%965=304%:%
%:%966=305%:%
%:%967=305%:%
%:%968=305%:%
%:%969=305%:%
%:%970=305%:%
%:%971=306%:%
%:%972=306%:%
%:%973=306%:%
%:%974=306%:%
%:%975=307%:%
%:%976=307%:%
%:%977=308%:%
%:%978=308%:%
%:%979=308%:%
%:%980=308%:%
%:%981=308%:%
%:%982=309%:%
%:%988=309%:%
%:%991=310%:%
%:%992=311%:%
%:%993=311%:%
%:%994=312%:%
%:%997=313%:%
%:%1001=313%:%
%:%1002=313%:%
%:%1003=313%:%
%:%1008=313%:%
%:%1011=314%:%
%:%1012=315%:%
%:%1013=315%:%
%:%1014=316%:%
%:%1021=317%:%
%:%1022=317%:%
%:%1023=318%:%
%:%1024=318%:%
%:%1025=319%:%
%:%1026=319%:%
%:%1027=320%:%
%:%1028=320%:%
%:%1029=321%:%
%:%1030=321%:%
%:%1031=321%:%
%:%1032=321%:%
%:%1033=322%:%
%:%1039=322%:%
%:%1042=323%:%
%:%1043=324%:%
%:%1044=324%:%
%:%1045=325%:%
%:%1046=326%:%
%:%1047=327%:%
%:%1048=327%:%
%:%1049=328%:%
%:%1050=329%:%
%:%1051=330%:%
%:%1054=331%:%
%:%1058=331%:%
%:%1059=331%:%
%:%1060=331%:%
%:%1061=331%:%
%:%1066=331%:%
%:%1069=332%:%
%:%1070=333%:%
%:%1071=333%:%
%:%1072=334%:%
%:%1073=335%:%
%:%1075=335%:%
%:%1079=335%:%
%:%1080=335%:%
%:%1081=335%:%
%:%1082=335%:%
%:%1089=335%:%
%:%1090=336%:%
%:%1091=337%:%
%:%1092=337%:%
%:%1093=338%:%
%:%1094=339%:%
%:%1095=340%:%
%:%1096=341%:%
%:%1103=342%:%
%:%1104=342%:%
%:%1105=343%:%
%:%1106=343%:%
%:%1107=344%:%
%:%1108=344%:%
%:%1109=344%:%
%:%1110=345%:%
%:%1111=345%:%
%:%1112=346%:%
%:%1113=346%:%
%:%1114=346%:%
%:%1115=347%:%
%:%1116=347%:%
%:%1117=347%:%
%:%1118=348%:%
%:%1119=348%:%
%:%1120=349%:%
%:%1121=349%:%
%:%1122=350%:%
%:%1123=350%:%
%:%1124=350%:%
%:%1125=351%:%
%:%1126=351%:%
%:%1127=352%:%
%:%1128=352%:%
%:%1129=352%:%
%:%1130=353%:%
%:%1131=353%:%
%:%1132=353%:%
%:%1133=354%:%
%:%1134=354%:%
%:%1135=354%:%
%:%1136=355%:%
%:%1137=355%:%
%:%1138=356%:%
%:%1139=356%:%
%:%1140=357%:%
%:%1141=357%:%
%:%1142=358%:%
%:%1143=358%:%
%:%1144=358%:%
%:%1145=359%:%
%:%1146=359%:%
%:%1147=359%:%
%:%1148=359%:%
%:%1149=360%:%
%:%1150=360%:%
%:%1151=360%:%
%:%1152=361%:%
%:%1153=361%:%
%:%1154=362%:%
%:%1155=362%:%
%:%1156=362%:%
%:%1157=363%:%
%:%1158=363%:%
%:%1159=364%:%
%:%1160=364%:%
%:%1161=364%:%
%:%1162=365%:%
%:%1163=365%:%
%:%1164=366%:%
%:%1165=366%:%
%:%1166=367%:%
%:%1167=367%:%
%:%1168=367%:%
%:%1169=368%:%
%:%1170=368%:%
%:%1171=368%:%
%:%1172=369%:%
%:%1173=369%:%
%:%1174=369%:%
%:%1175=369%:%
%:%1176=369%:%
%:%1177=370%:%
%:%1178=370%:%
%:%1179=371%:%
%:%1180=371%:%
%:%1181=371%:%
%:%1182=371%:%
%:%1183=371%:%
%:%1184=372%:%
%:%1185=372%:%
%:%1186=373%:%
%:%1187=373%:%
%:%1188=374%:%
%:%1189=374%:%
%:%1190=374%:%
%:%1191=374%:%
%:%1192=374%:%
%:%1193=375%:%
%:%1199=375%:%
%:%1202=376%:%
%:%1203=377%:%
%:%1204=377%:%
%:%1205=378%:%
%:%1216=389%:%
%:%1223=390%:%
%:%1224=390%:%
%:%1225=391%:%
%:%1226=391%:%
%:%1227=392%:%
%:%1228=392%:%
%:%1229=392%:%
%:%1230=392%:%
%:%1231=393%:%
%:%1232=393%:%
%:%1233=394%:%
%:%1234=394%:%
%:%1235=395%:%
%:%1236=395%:%
%:%1237=395%:%
%:%1238=395%:%
%:%1239=395%:%
%:%1240=396%:%
%:%1241=396%:%
%:%1242=397%:%
%:%1243=397%:%
%:%1244=398%:%
%:%1245=398%:%
%:%1246=398%:%
%:%1247=398%:%
%:%1248=398%:%
%:%1249=399%:%
%:%1255=399%:%
%:%1258=400%:%
%:%1259=401%:%
%:%1260=401%:%
%:%1261=402%:%
%:%1262=403%:%
%:%1263=404%:%
%:%1264=404%:%
%:%1267=405%:%
%:%1271=405%:%
%:%1272=405%:%
%:%1273=405%:%
%:%1278=405%:%
%:%1281=406%:%
%:%1282=407%:%
%:%1283=407%:%
%:%1284=408%:%
%:%1285=409%:%
%:%1292=410%:%
%:%1293=410%:%
%:%1294=411%:%
%:%1295=411%:%
%:%1296=412%:%
%:%1297=412%:%
%:%1298=412%:%
%:%1299=413%:%
%:%1300=413%:%
%:%1301=413%:%
%:%1302=413%:%
%:%1303=414%:%
%:%1304=414%:%
%:%1305=414%:%
%:%1306=414%:%
%:%1307=415%:%
%:%1308=415%:%
%:%1309=415%:%
%:%1310=416%:%
%:%1311=416%:%
%:%1312=417%:%
%:%1313=417%:%
%:%1314=417%:%
%:%1315=417%:%
%:%1316=417%:%
%:%1317=418%:%
%:%1318=418%:%
%:%1319=418%:%
%:%1320=418%:%
%:%1321=419%:%
%:%1322=419%:%
%:%1323=419%:%
%:%1324=419%:%
%:%1325=419%:%
%:%1326=420%:%
%:%1327=420%:%
%:%1328=420%:%
%:%1329=421%:%
%:%1330=421%:%
%:%1331=421%:%
%:%1332=422%:%
%:%1333=422%:%
%:%1334=422%:%
%:%1335=422%:%
%:%1336=422%:%
%:%1337=423%:%
%:%1347=425%:%
%:%1348=426%:%
%:%1349=427%:%
%:%1351=428%:%
%:%1352=428%:%
%:%1353=429%:%
%:%1354=430%:%
%:%1361=431%:%
%:%1362=431%:%
%:%1363=432%:%
%:%1364=432%:%
%:%1365=432%:%
%:%1366=433%:%
%:%1367=433%:%
%:%1368=434%:%
%:%1369=434%:%
%:%1370=435%:%
%:%1371=436%:%
%:%1372=436%:%
%:%1373=436%:%
%:%1374=437%:%
%:%1375=438%:%
%:%1376=438%:%
%:%1377=438%:%
%:%1378=439%:%
%:%1379=439%:%
%:%1380=439%:%
%:%1381=439%:%
%:%1382=440%:%
%:%1383=440%:%
%:%1384=440%:%
%:%1385=441%:%
%:%1386=441%:%
%:%1387=441%:%
%:%1388=442%:%
%:%1389=443%:%
%:%1390=443%:%
%:%1391=443%:%
%:%1392=444%:%
%:%1393=444%:%
%:%1394=445%:%
%:%1395=445%:%
%:%1396=445%:%
%:%1397=445%:%
%:%1398=446%:%
%:%1399=446%:%
%:%1400=446%:%
%:%1401=446%:%
%:%1402=447%:%
%:%1403=447%:%
%:%1404=447%:%
%:%1405=447%:%
%:%1406=447%:%
%:%1407=448%:%
%:%1408=448%:%
%:%1409=448%:%
%:%1410=448%:%
%:%1411=448%:%
%:%1412=449%:%
%:%1413=449%:%
%:%1414=449%:%
%:%1415=449%:%
%:%1416=449%:%
%:%1417=450%:%
%:%1427=452%:%
%:%1429=453%:%
%:%1430=453%:%
%:%1431=454%:%
%:%1432=455%:%
%:%1439=456%:%
%:%1440=456%:%
%:%1441=457%:%
%:%1442=457%:%
%:%1443=458%:%
%:%1444=458%:%
%:%1445=458%:%
%:%1446=459%:%
%:%1447=459%:%
%:%1448=459%:%
%:%1449=459%:%
%:%1450=460%:%
%:%1451=460%:%
%:%1452=460%:%
%:%1453=460%:%
%:%1454=461%:%
%:%1460=461%:%
%:%1463=462%:%
%:%1464=463%:%
%:%1465=463%:%
%:%1466=464%:%
%:%1467=465%:%
%:%1470=466%:%
%:%1474=466%:%
%:%1475=466%:%
%:%1476=467%:%
%:%1477=467%:%
%:%1478=468%:%
%:%1479=468%:%
%:%1480=469%:%
%:%1481=469%:%
%:%1482=469%:%
%:%1483=470%:%
%:%1484=470%:%
%:%1485=471%:%
%:%1486=471%:%
%:%1487=471%:%
%:%1488=471%:%
%:%1489=471%:%
%:%1490=472%:%
%:%1491=472%:%
%:%1492=473%:%
%:%1493=473%:%
%:%1494=474%:%
%:%1495=474%:%
%:%1496=474%:%
%:%1497=474%:%
%:%1498=475%:%
%:%1499=475%:%
%:%1500=475%:%
%:%1501=475%:%
%:%1502=476%:%
%:%1503=476%:%
%:%1504=477%:%
%:%1505=477%:%
%:%1510=477%:%
%:%1513=478%:%
%:%1514=479%:%
%:%1515=479%:%
%:%1516=480%:%
%:%1517=481%:%
%:%1520=482%:%
%:%1524=482%:%
%:%1525=482%:%
%:%1526=483%:%
%:%1527=483%:%
%:%1528=484%:%
%:%1529=484%:%
%:%1530=485%:%
%:%1531=485%:%
%:%1532=485%:%
%:%1533=486%:%
%:%1534=486%:%
%:%1535=487%:%
%:%1536=487%:%
%:%1537=487%:%
%:%1538=487%:%
%:%1539=487%:%
%:%1540=488%:%
%:%1541=488%:%
%:%1542=489%:%
%:%1543=489%:%
%:%1544=490%:%
%:%1545=490%:%
%:%1546=490%:%
%:%1547=490%:%
%:%1548=491%:%
%:%1549=491%:%
%:%1550=492%:%
%:%1551=492%:%
%:%1552=492%:%
%:%1553=493%:%
%:%1554=493%:%
%:%1555=494%:%
%:%1556=494%:%
%:%1561=494%:%
%:%1564=495%:%
%:%1565=496%:%
%:%1566=496%:%
%:%1567=497%:%
%:%1570=500%:%
%:%1571=501%:%
%:%1572=502%:%
%:%1573=502%:%
%:%1574=503%:%
%:%1575=504%:%
%:%1576=505%:%
%:%1577=506%:%
%:%1580=507%:%
%:%1584=507%:%
%:%1585=507%:%
%:%1586=507%:%
%:%1587=507%:%
%:%1592=507%:%
%:%1595=508%:%
%:%1596=509%:%
%:%1597=509%:%
%:%1598=510%:%
%:%1599=511%:%
%:%1600=512%:%
%:%1601=513%:%
%:%1602=514%:%
%:%1605=515%:%
%:%1609=515%:%
%:%1610=515%:%
%:%1611=515%:%
%:%1612=515%:%
%:%1617=515%:%
%:%1620=516%:%
%:%1621=517%:%
%:%1622=517%:%
%:%1623=518%:%
%:%1624=519%:%
%:%1625=520%:%
%:%1626=521%:%
%:%1633=522%:%
%:%1634=522%:%
%:%1635=523%:%
%:%1636=523%:%
%:%1637=523%:%
%:%1638=524%:%
%:%1639=524%:%
%:%1640=524%:%
%:%1641=525%:%
%:%1642=525%:%
%:%1643=526%:%
%:%1644=526%:%
%:%1645=526%:%
%:%1646=527%:%
%:%1647=527%:%
%:%1648=527%:%
%:%1649=528%:%
%:%1650=528%:%
%:%1651=529%:%
%:%1652=529%:%
%:%1653=530%:%
%:%1654=530%:%
%:%1655=530%:%
%:%1656=531%:%
%:%1657=531%:%
%:%1658=532%:%
%:%1659=532%:%
%:%1660=532%:%
%:%1661=533%:%
%:%1662=533%:%
%:%1663=533%:%
%:%1664=534%:%
%:%1665=534%:%
%:%1666=534%:%
%:%1667=535%:%
%:%1668=535%:%
%:%1669=536%:%
%:%1670=536%:%
%:%1671=537%:%
%:%1672=537%:%
%:%1673=538%:%
%:%1674=538%:%
%:%1675=538%:%
%:%1676=539%:%
%:%1677=539%:%
%:%1678=539%:%
%:%1679=539%:%
%:%1680=540%:%
%:%1681=540%:%
%:%1682=540%:%
%:%1683=541%:%
%:%1684=541%:%
%:%1685=542%:%
%:%1686=542%:%
%:%1687=542%:%
%:%1688=543%:%
%:%1689=543%:%
%:%1690=544%:%
%:%1691=544%:%
%:%1692=544%:%
%:%1693=545%:%
%:%1694=545%:%
%:%1695=546%:%
%:%1696=546%:%
%:%1697=547%:%
%:%1698=547%:%
%:%1699=547%:%
%:%1700=548%:%
%:%1701=548%:%
%:%1702=549%:%
%:%1703=549%:%
%:%1704=550%:%
%:%1705=550%:%
%:%1706=550%:%
%:%1707=550%:%
%:%1708=550%:%
%:%1709=551%:%
%:%1710=551%:%
%:%1711=552%:%
%:%1712=552%:%
%:%1713=552%:%
%:%1714=552%:%
%:%1715=552%:%
%:%1716=553%:%
%:%1717=553%:%
%:%1718=554%:%
%:%1719=554%:%
%:%1720=555%:%
%:%1721=555%:%
%:%1722=556%:%
%:%1723=556%:%
%:%1724=556%:%
%:%1725=557%:%
%:%1726=557%:%
%:%1727=557%:%
%:%1728=557%:%
%:%1729=557%:%
%:%1730=558%:%
%:%1731=558%:%
%:%1732=559%:%
%:%1733=559%:%
%:%1734=560%:%
%:%1735=560%:%
%:%1736=560%:%
%:%1737=560%:%
%:%1738=561%:%
%:%1739=561%:%
%:%1740=562%:%
%:%1741=562%:%
%:%1742=562%:%
%:%1743=562%:%
%:%1744=563%:%
%:%1745=564%:%
%:%1746=564%:%
%:%1747=564%:%
%:%1748=565%:%
%:%1749=565%:%
%:%1750=566%:%
%:%1751=566%:%
%:%1752=566%:%
%:%1753=567%:%
%:%1754=568%:%
%:%1755=568%:%
%:%1756=568%:%
%:%1757=569%:%
%:%1758=569%:%
%:%1759=569%:%
%:%1760=570%:%
%:%1761=570%:%
%:%1762=570%:%
%:%1763=571%:%
%:%1764=571%:%
%:%1765=571%:%
%:%1766=571%:%
%:%1767=572%:%
%:%1768=572%:%
%:%1769=572%:%
%:%1770=573%:%
%:%1771=573%:%
%:%1772=573%:%
%:%1773=574%:%
%:%1774=574%:%
%:%1775=575%:%
%:%1776=575%:%
%:%1777=575%:%
%:%1778=575%:%
%:%1779=576%:%
%:%1780=576%:%
%:%1781=577%:%
%:%1782=577%:%
%:%1783=578%:%
%:%1784=579%:%
%:%1785=580%:%
%:%1786=580%:%
%:%1787=580%:%
%:%1788=580%:%
%:%1789=580%:%
%:%1790=581%:%
%:%1796=581%:%
%:%1799=582%:%
%:%1800=583%:%
%:%1801=583%:%
%:%1802=584%:%
%:%1813=595%:%
%:%1820=596%:%
%:%1821=596%:%
%:%1822=597%:%
%:%1823=597%:%
%:%1824=598%:%
%:%1825=598%:%
%:%1826=598%:%
%:%1827=598%:%
%:%1828=599%:%
%:%1829=599%:%
%:%1830=600%:%
%:%1831=600%:%
%:%1832=601%:%
%:%1833=601%:%
%:%1834=601%:%
%:%1835=601%:%
%:%1836=601%:%
%:%1837=602%:%
%:%1838=602%:%
%:%1839=603%:%
%:%1840=603%:%
%:%1841=604%:%
%:%1842=604%:%
%:%1843=604%:%
%:%1844=604%:%
%:%1845=604%:%
%:%1846=605%:%
%:%1852=605%:%
%:%1855=606%:%
%:%1856=607%:%
%:%1857=607%:%
%:%1860=608%:%
%:%1865=609%:%
%:%1873=609%:%

==> LaTeXsugar.tex <==
\endinput
%:%file=~/Productions/articles/ijcar2020/LMCS/LaTeXsugar.thy%:%

==> session.tex <==
\input{LaTeXsugar.tex}
\input{Paper_VC.tex}
\input{Paper_SC.tex}
\input{Paper_MIS.tex}
\input{Paper_LB.tex}
\input{Paper_CS.tex}
\input{Paper_BP.tex}

